UAV-assisted Online Machine Learning over Multi-Tiered Networks: A Hierarchical Nested Personalized Federated Learning Approach

We investigate training machine learning (ML) models across a set of geo-distributed, resource-constrained clusters of devices through unmanned aerial vehicles (UAV) swarms. The presence of time-varying data heterogeneity and computational resource inadequacy among device clusters motivate four key parts of our methodology: (i) stratified UAV swarms of leader, worker, and coordinator UAVs, (ii) hierarchical nested personalized federated learning (HN-PFL), a distributed ML framework for personalized model training across the worker-leader-core network hierarchy, (iii) cooperative UAV resource pooling to address computational inadequacy of devices by conducting model training among the UAV swarms, and (iv) model/concept drift to model time-varying data distributions. In doing so, we consider both micro (i.e., UAV-level) and macro (i.e., swarm-level) system design. At the micro-level, we propose network-aware HN-PFL, where we distributively orchestrate UAVs inside swarms to optimize energy consumption and ML model performance with performance guarantees. At the macro-level, we focus on swarm trajectory and learning duration design, which we formulate as a sequential decision making problem tackled via deep reinforcement learning. Our simulations demonstrate the improvements achieved by our methodology in terms of ML performance, network resource savings, and swarm trajectory efficiency.

==> HN-PFL_algo.tex <==

% \begin{algorithm}[t]
% \footnotesize
% \SetAlgoLined
% %\KwResult{HN-PFL}
% Set Initial = True; \\
% \henry{fix later}
%  Initialize $\mathbf{w}^{\textsf{init}}$ at $AP$;\\
% \If{Initial == True}{
%     $\mathbf{w}^u(0) \leftarrow \mathbf{w}^{\textsf{init}}, \forall u \in \mathcal{U}$;\\
%     % $\mathbf{w}^{i}(0) \leftarrow \mathbf{w}^u(0), \forall i \in \cup_{u \in \mathcal{U}} \mathcal{U}_u$; \\
%     }
%  \While{System Operational}{
%  Set $t = 1$, $K_2 = \floor{\frac{T}{\tau_2}}$; \\

%  Determine $\tau_1$, $\tau_2$ based on~\eqref{eq:f1_obj};\\
 
%  \For{$k_2 \in \{1, \cdots, K_2\}$}{
%     % \Else{
%     % $\mathbf{w}^u(k_2\tau_2) \leftarrow \mathbf{w}(k_2\tau_2), \forall u \in \mathcal{U}$; \\
%     % % $\mathbf{w}^{i}(k_2 \tau_2) \leftarrow \mathbf{w}^{u}(k_2 \tau_2), \forall i \in \cup_{u \in \mathcal{U}}\mathcal{U}_u$; \\
%     % }
    
%     \For{$k_1 \in \{1, \cdots, \tau_2\}$}{
%     \henry{need to indicate comment}
%     $\doublearraybackslash$ Local synchronization $\mathbf{w}^{i}(k_1 \tau_1) \leftarrow \mathbf{w}^{u}(k_1 \tau_1), \forall i \in \cup_{u \in \mathcal{U}}\mathcal{U}_u$; \\
%     \For{$i \in \mathcal{W}_u(t)$}{
%     \For{$t \in \{\tau_1 (k_1-1)+1, \cdots, \tau_1 k_1 \}$}{
%     Compute local meta-gradient, $\widetilde{\nabla F_i}(t-1)$, with independent batches $\mathcal{D}_i^1$, $\mathcal{D}_i^2$, and $\mathcal{D}_i^3$; \\
%     Update model parameters: $\mathbf{w}^i(t) = \mathbf{w}^i(t-1) - \eta_2 \widetilde{\nabla F_i}(t-1)$ as in~\eqref{eq:pfl_combined_minibatches}; \\ 
%     }
%     }
%     Local aggregation $\mathbf{w}^{u}(\tau_1 k_1) = \frac{1}{W_u(t)} \sum_{i \in \mathcal{W}_u(t)} \mathbf{w}^{i}(\tau_1 k_1)$; \\ 
%     Local re-synchronization $\mathbf{w}^{i}(\tau_1 k_1) \leftarrow \mathbf{w}^{u}(\tau_1 k_1), \forall i \in \mathcal{W}_u(t)$; \\
%     }
%     Global aggregation $\mathbf{w}(\tau_2 k_2) = \frac{1}{U} \sum_{u \in \mathcal{U}} \mathbf{w}^{u}(\tau_2 k_2)$; \\
%     Global re-synchronization $\mathbf{w}^{u}(\tau_2 k_2) \leftarrow \mathbf{w}(\tau_2 k_2)$; \\
%     }
 
%  \For{$u \in \mathcal{U}$}{
%   Local re-synchronization $\mathbf{w}^{i}(\tau_1 k_1) \leftarrow \mathbf{w}^{u}(\tau_1 k_1), \forall i \in \mathcal{W}_u(t)$; \\
%  \For{$i \in \mathcal{W}_u(t)$}{
%  \For{$t \in \{T+1, \cdots, T+T_p\}$}{
%     Compute local meta-gradient, $\widetilde{\nabla F_i}(t-1)$, with independent batches $\mathcal{D}_i^1$, $\mathcal{D}_i^2$, and $\mathcal{D}_i^3$; \\
%     Update model parameters: $\mathbf{w}^i(t) = \mathbf{w}^i(t-1) - \eta_2 \widetilde{\nabla F_i}(t-1)$ as in~\eqref{eq:pfl_combined_minibatches}; \\ 
%  }
%  }
%      Local aggregation $\mathbf{w}^{u}(\tau_1 k_1) = \frac{1}{W_u(t)} \sum_{i \in \mathcal{W}_u(t)} \mathbf{w}^{i}(\tau_1 k_1)$; \\ 
%     Local re-synchronization $\mathbf{w}^{i}(\tau_1 k_1) \leftarrow \mathbf{w}^{u}(\tau_1 k_1), \forall i \in \mathcal{W}_u(t)$; \\
%  }
%  }
%  \caption{To be written}
% \label{alg:hnpfl}
% \end{algorithm}

==> graveyard.tex <==
%% -- Math notation from Overarching Optimization --
%\frac{F_m(w_m(t) \vert \mathcal{D}_m(t))}{D_m(t)}
%E^{c}_{\mathcal{U}_u}
%\int_{t-1}^{t} \left[ c_1 \Vert v_u(\tau) \Vert ^3 + \frac{c_2}{\Vert v_u(\tau) \Vert} (1 + \frac{\Vert a_u(\tau) \Vert^2 - \frac{(a_u(\tau)v_u(\tau))^2}{\Vert v_u(\tau) \Vert^2}}{g^2}) \right] dt 




%% -- Ideas list for overarching optimization --
\iffalse
-- trajectory specific
How to embed the data collection optimization within the trajectory optimization?
Objective: 
a) travel power used
b) optimize swaps of coordination/storage UAVs?!
make constraint - if cost in energy greater than expected gain in performance, then don't move; else move, the number of moving UAVs is embedded in this inequality
This will need to be a theorem: we quantify the relationship amon UAV device capabilities/total swarm capabilities + underlying data quality to loss and performance of an ML model
c) re-charging points (position of re-charging points)
constraint - expected power consumption + energy to nearest recharge location <= current battery
d) online aggregate envrionment loss
e) prioritize revisits to sensors with high underlying distribution change
f) embed the local device cluster minimization problem within
\fi

%% -- Amazon Sidewalk paragraphs--
%While distant and distinct communities are unlikely to be connected to each other, their classification goals are likely to rely on the same underlying data/images with slight deviations. For example, for neighborhood safety, a people/property classifying ML model based on smart home sensors and cameras could be trained. 

%There are three problems preventing such classification models from scaling up: (i) home devices may not be idle or plugged into a constant source of power - therefore preventing home IoT devices from performing ML training locally, (ii) distant neighborhoods are not connected but may have similar model needs, and (iii) neighborhoods change over time - i.e., the underlying data distributions are online.











% ## notation table figments

%$\mathcal{G}^{\mathcal{C}_n}$ & Network Graph for Device Cluster $n$
% $\mathcal{G}$ & Network Graph for Overarching Environment
% & & & & \\
% \midrule

% \multicolumn{2}{c}{\textbf{Device and UAV Notation and Energy Consumption}}\\
% $\rho_{i,j}(t)$ & Ratio of Data Transfer from device $i$ to UAV $j$\\
% $\varrho_{i,j}(t)$ & Ratio of Data Transfer from UAV $i$ to UAV $j$\\
% $\widetilde{\phi^{m}_{i,j}}(t)$ & Bandwidth cost from device $i$ to UAV $j$ in swarm $\mathcal{U}_m(t)$\\
% $\phi^{m}_{i,j}(t)$ & Bandwidth cost from UAV $i$ to UAV $j$ in swarm $\mathcal{U}_m(t)$\\
% $\Phi^{m}_{j}(t)$ & Bandwidth limit for UAV $j$ in swarm $\mathcal{U}_m$\\
% $c_j$ & CPU cost per processed datum at UAV $j$\\
% $f_j(t)$ & Adjustable CPU cycle frequency at UAV $j$\\
% $s_j(t)$ & Ratio of Data to Process at UAV $j$\\
% $u_j(t)$ & Coordination/storage UAV flag at $j$\\
% $E^{p}_{j}(t)$ & Energy used to Process Data at $j$-th UAV \\ 
% $E^{c}_{j}(t)$ & Energy used to Commute for $j$-th UAV \\
% $E^{tx,\mathcal{C}_m}_{j}(t)$ & Energy used to Transmit Data by $j$-th Device in $\mathcal{C}_m$\\
% $E^{tx,\widetilde{\mathcal{U}}_m}_{j}(t)$ & Energy used to Transmit Data by $j$-th UAV in $\widetilde{\mathcal{U}}_m$\\
% $E^{b}_{j}(t)$ & Battery Energy at UAV $j$\\
% $\Psi^{p}_j(t)$ & Max Energy for Data Processing at $j$-th UAV\\
% $\Psi^{c}_j(t)$ & Max Energy for Commuting at $j$-th UAV\\
% $\Psi^{\mathcal{C}_m}_{j}(t)$ & Max Energy for Transmitting at $j$-th Device in $\mathcal{C}_m$\\
% $\Psi^{\widetilde{\mathcal{U}}_m}_{j}(t)$ & Max energy for Transmitting at $j$-th UAV in $\widetilde{\mathcal{U}}_m$ \\

% \midrule

% \multicolumn{2}{c}{\textbf{Network Notation}} & \multicolumn{2}{c}{\textbf{ML Notation}} \\
% $\mathcal{G}^{\mathcal{C}_n}$ & Network Graph for Device Cluster $n$\\
% $\mathcal{G}$ & Network Graph for Overarching Environment\\
% \midrule
% \multicolumn{2}{c}{\textbf{ML Notation}}\\
% F & Model Loss \\
% $\mathbf{w}^{\mathcal{C}_i}_j(t)$ & Model Parameters at UAV $j$ for device cluster $\mathcal{C}_i$\\
% $\mathbf{w}^{\mathcal{C}_i}_{\mathcal{U}_m}(t)$ & Aggregated Model Parameters at swarm $\mathcal{U}_m$ for cluster $\mathcal{C}_i$ \\
% $\mathbf{w}^{\mathcal{C}_i}(t)$ & Global, Personalized Model Parameters for cluster $\mathcal{C}_i$\\
% \bottomrule

==> l1_proof.tex <==

\begin{proof}
We first recall the definition of the approximated meta-gradient:
\begin{equation} \label{eq:proof_l1_meta_grad}
\begin{aligned}
\widetilde{\nabla F_i}(\mathbf{w}) = (\mathbf{I} - \eta_1 \widetilde{\nabla^2 L_i}(\mathbf{w}, \mathcal{D}_{i}^{'''}(t) )) \widetilde{\nabla L_i} (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_{i}^{'}(t)),\mathcal{D}_{i}^{''}(t)),
\end{aligned}
\end{equation}

where $\mathcal{D}_{i}^{'}(t)$,  $\mathcal{D}_{i}^{''}(t)$, and $\mathcal{D}_{i}^{'''}(t)$ are defined as  $\alpha_1^{u}(t) \mathcal{D}_{i}(t)$, $\alpha_2^{u}(t) \mathcal{D}_{i}(t)$, and $\alpha_3^{u}(t) \mathcal{D}_{i}(t)$ respectively. Additionally, we note that the datasets $\mathcal{D}_{i}^{'}(t)$,  $\mathcal{D}_{i}^{''}(t)$, and $\mathcal{D}_{i}^{'''}(t)$ are sampled uniformly at random and with replacement from $\mathcal{D}_i(t)$.

We re-express~\eqref{eq:proof_l1_meta_grad} using the true gradients, obtaining:

\begin{equation}
\begin{aligned}
&\widetilde{\nabla F_i}(\mathbf{w}) = \bigg(\mathbf{I} - \eta_1 \bigg[ \widetilde{\nabla^2 L_i}(\mathbf{w}, \mathcal{D}_{i}^{'''}(t) ) +\nabla^2 L_i(\mathbf{w}) - \nabla^2 L_i(\mathbf{w}) \bigg] \bigg) \bigg[\widetilde{\nabla L_i} (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_{i}^{'}(t)),\mathcal{D}_{i}^{''}(t)) \\
&+ \nabla L_i (\mathbf{w} - \eta_1 \nabla L_i(\mathbf{w})) - \nabla L_i (\mathbf{w} - \eta_1 \nabla L_i(\mathbf{w}))  \bigg].
\end{aligned}
\end{equation}

For simplicity of analysis, we now define two auxiliary variables:

\begin{equation}
\begin{aligned}
& e_1 = \eta_1 (\nabla^2 L_i(\mathbf{w}) - \widetilde{\nabla^2 L_i}(\mathbf{w}, \mathcal{D}_{i}^{'''}(t) )) \\
& e_2 = \widetilde{\nabla L_i} (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_{i}^{'}(t)),\mathcal{D}_{i}^{''}(t)) - \nabla L_i (\mathbf{w} - \eta_1 \nabla L_i(\mathbf{w})) \\
&+ \nabla L_i (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_i^{'}(t))) - \nabla L_i (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_i^{'}(t))).
\end{aligned}
\end{equation}

Using our assumption~\ref{eq:assumption_stochastic_gradient_sigma}, we simplify $e_1$ as:

\begin{equation}
\begin{aligned}
& \mathbb{E}\bigg[\Vert e_1 \Vert^2 \bigg] \leq \eta_1^2 \frac{(\sigma_{H}^{u})^2}{D_{i}^{'''}(t)},
\end{aligned}
\end{equation}

and $e_2$ as: 

\begin{equation}
\begin{aligned}
& \mathbb{E}\bigg[\Vert e_2 \Vert^2 \bigg] = \mathbb{E}\bigg[\mathbb{E}\bigg[\Vert e_2 \Vert^2 \vert \mathcal{D}_i^{'}(t) \bigg]\bigg] \\
& = \mathbb{E}\bigg[ \Vert \widetilde{\nabla L_i} (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_{i}^{'}(t)),\mathcal{D}_{i}^{''}(t)) 
 - \nabla L_i (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_i^{'}(t))) \Vert^2 \bigg]\\
 & + \mathbb{E} \bigg[ \Vert \nabla L_i (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_i^{'}(t))) 
- \nabla L_i (\mathbf{w} - \eta_1 \nabla L_i(\mathbf{w}))  \Vert^2 \bigg] \\
& \leq \frac{(\sigma_{G}^{u})^2}{D_{i}^{''}(t)} + \mu^2 \eta_1^2 \mathbb{E}\bigg[\Vert  \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_i^{'}(t)) - \nabla L_i(\mathbf{w}) \Vert^2 \bigg] \\
& \leq \frac{(\sigma_{G}^{u})^2}{D_{i}^{''}(t)} + \frac{\mu^2 \eta_1^2 (\sigma_{G}^{u})^2}{D_{i}^{'}(t)}.
\end{aligned}
\end{equation}

Now, we find a bound for $\mathbb{E}\bigg[\Vert \widetilde{\nabla F_i}(\mathbf{w}) - \nabla F_i(\mathbf{w}) \Vert^2\bigg]$. First, we note that: 

\begin{equation}
\begin{aligned}
\Vert \widetilde{\nabla F_i}(\mathbf{w}) - \nabla F_i(\mathbf{w}) \Vert \leq \Vert \mathbf{I} - \eta_1 \nabla^2 L_i(\mathbf{w}) \Vert \Vert e_2 \Vert + \Vert e_1 \Vert \Vert \nabla L_i(\mathbf{w} - \eta_1 \nabla L_i(\mathbf{w})) \Vert + \Vert e_1 \Vert \Vert e_2 \Vert,
\end{aligned}
\end{equation}

then, using Cauchy-Schwarz as $(a+b+c)^2 \leq 3(a^2 + b^2 + c^2)$ gives: %with $a,b,c \geq 0$ gives:

\begin{equation}
\begin{aligned}
\Vert \widetilde{\nabla F_i}(\mathbf{w}) - \nabla F_i(\mathbf{w}) \Vert^2 \leq 3\Vert \mathbf{I} - \eta_1 \nabla^2 L_i(\mathbf{w}) \Vert^2 \Vert e_2 \Vert^2 + 3\Vert e_1 \Vert^2 \Vert \nabla L_i(\mathbf{w} - \eta_1 \nabla L_i(\mathbf{w})) \Vert^2 + 3\Vert e_1 \Vert^2 \Vert e_2 \Vert^2.
\end{aligned}
\end{equation}

Next, since $\Vert \mathbf{I} - \eta_1 \nabla^2 L_i(\mathbf{w})\Vert \leq 1 + \eta_1 \mu \leq 2$ as $\eta_1 \in (0,\frac{1}{\mu}]$ and $\Vert \nabla L_i(\mathbf{w}) \Vert \leq B$, we have:

\begin{equation}
\begin{aligned}
&\mathbb{E}\bigg[ \Vert \widetilde{\nabla F_i}(\mathbf{w}) - \nabla F_i(\mathbf{w}) \Vert^2 \bigg] \leq 3B^2 \mathbb{E}[\Vert e_1 \Vert^2] + 12 \mathbb{E}[\Vert e_2 \Vert^2] + 3 \mathbb{E}[\Vert e_1 \Vert^2]  \mathbb{E}[\Vert e_2 \Vert^2] \\
& \leq (\sigma_F^i)^2 \triangleq 3 B^2 \eta_1^2 \frac{(\sigma_H^{u})^2}{D_i^{'''}(t)} + 12 \frac{(\sigma_{G}^{u})^2}{D_{i}^{''}(t)} + \frac{\mu^2 \eta_1^2 (\sigma_{G}^{u})^2}{D_{i}^{'}(t)} + 3 \eta_1^2 \frac{(\sigma_H^{u})^2}{D_i^{'''}(t)} \bigg(\frac{(\sigma_{G}^{u})^2}{D_{i}^{''}(t)} + \frac{\mu^2 \eta_1^2 (\sigma_{G}^{u})^2}{D_{i}^{'}(t)}\bigg),
\end{aligned}
\end{equation}

which is the result.

% \begin{equation} \label{eq:e2_raw}
% \begin{aligned}
% & \mathbb{E}\bigg[\Vert e_2 \Vert^2 \bigg] \leq \mathbb{E}\bigg[ \Vert \widetilde{\nabla L_i} (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_{i}^{'}(t)),\mathcal{D}_{i}^{''}(t)) 
%  - \nabla L_i (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_i^{'}(t))) \\
% &+ \nabla L_i (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_i^{'}(t))) 
% - \nabla L_i (\mathbf{w} - \eta_1 \nabla L_i(\mathbf{w}))  \Vert^2 \bigg].
% \end{aligned}
% \end{equation}

% Since the first term on the right hand side in~\eqref{eq:e2_raw} has zero mean,~\eqref{eq:e2_raw} becomes:

% \begin{equation}
% \begin{aligned}
% & \mathbb{E}\bigg[\Vert e_2 \Vert^2 \bigg] \leq \mathbb{E} \bigg[ \Vert \nabla L_i (\mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_i^{'}(t))) 
% - \nabla L_i (\mathbf{w} - \eta_1 \nabla L_i(\mathbf{w}))  \Vert^2 \bigg] \\
% &\leq \hat{\mu_i} \mathbb{E}\bigg[\Vert \mathbf{w} - \eta_1 \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_i^{'}(t)) - \mathbf{w} + \eta_1 \nabla L_i(\mathbf{w}) \Vert\bigg] \\
% & = \hat{\mu_i} \eta_1 \mathbb{E}\bigg[\Vert \nabla L_i(\mathbf{w}) - \widetilde{\nabla L_i}(\mathbf{w},\mathcal{D}_i^{'}(t))\Vert\bigg] \\
% & \leq \hat{\mu_i} \eta_1 \frac{(\sigma_{G}^{u})^2}{\sqrt{D_{i}^{'}(t)}},
% \end{aligned}
% \end{equation}

% and:

% \begin{equation}
% \mathbb{E}\bigg[\Vert e_2 \Vert^2 \bigg] \leq \hat{\mu_i}^2\eta_1^2 \frac{(\sigma_{G}^{u})^2}{\sqrt{D_{i}^{'}(t)}}.
% \end{equation}

\end{proof}

==> math_graveyard.tex <==
Then:
\begin{equation}
\begin{aligned}
&\mathbb{E} \bigg[\Vert w_{k_1}^{i}(t) - \frac{1}{W_u}\sum_{i\in \mathcal{W}_u} w_{k_1}^{i}(t) \Vert \bigg] \\
&= \mathbb{E} \bigg[\Vert w_{k_1}^{i}(t-1) - \beta \widetilde{\nabla}F_i(w_{k_1}^{i}(t-1)) \\
&-\frac{1}{W_u} \sum_{i\in \mathcal{W}_u}(w_{k_1}^{i}(t-1) - \beta \widetilde{\nabla}F_i(w_{k_1}^{i}(t-1))) \Vert\bigg] \\
&\leq \mathbb{E} \bigg[\Vert w_{k_1}^{i}(t-1) - \frac{1}{W_u}\sum_{i \in \mathcal{W}_u}w_{k_1}^{i}(t-1) \Vert\bigg] \\
&+ \beta \mathbb{E} \bigg[\Vert \widetilde{\nabla}F_i(w_{k_1}^{i}(t-1)) - \frac{1}{W_u}\sum_{i\in \mathcal{W}_u}\widetilde{\nabla}F_i(w_{k_1}^{i}(t-1)) \Vert\bigg].
\end{aligned}
\end{equation}

Next, we analyze the second term in the above inequality using similar techniques as proposition 1 from~\cite{temp}:
\begin{equation}
\begin{aligned}
&\beta \mathbb{E} \bigg[\Vert \widetilde{\nabla}F_i(w_{k_1}^{i}(t-1)) - \frac{1}{W_u}\sum_{i\in \mathcal{W}_u}\widetilde{\nabla}F_i(w_{k_1}^{i}(t-1)) \Vert\bigg] \\
& \leq \beta \mathbb{E} \bigg[\Vert \nabla F_i(w_{k_1}^{i}(t-1)) - \frac{1}{W_u}\sum_{i \in \mathcal{W}_u}\nabla F_i(w_{k_1}^{i}(t-1))\Vert \bigg] \\
&+ \beta \mathbb{E} \bigg[\Vert \nabla F_i(w_{k_1}^{i}(t-1)) - \widetilde{\nabla}F_i(w_{k_1}^{i}(t-1))\Vert \bigg] \\
&+ \frac{\beta}{W_u}\mathbb{E} \bigg[\Vert \sum_{i\in \mathcal{W}_u} (\nabla F_i(w_{k_1}^{i}(t-1)) - \widetilde{\nabla}F_i(w_{k_1}^{i}(t-1))) \Vert\bigg] \\
& \leq \beta \mathbb{E} \bigg[\Vert \nabla F_i(w_{k_1}^{i}(t-1)) - \frac{1}{W_u}\sum_{i \in \mathcal{W}_u}\nabla F_i(w_{k_1}^{i}(t-1))\Vert \bigg] \\
& + 2\beta \sigma_{F}^{u}
\end{aligned}
\end{equation}



% \begin{algorithm}
% \footnotesize
% \SetAlgoLined
% \KwResult{Sequential FL-PFL}
%  initialization\;
%  \While{$k_g \leq K_g$}{
%  \For{$\mathcal{U}_i(t) \in \mathcal{U}$}{
%  \For{$t \in \{\tau_s k_g +1, \cdots, \tau_s (k_g+1)\} $}{
%  \For{$j \in \mathcal{U}_i(t)$}{
%  $w^{\mathcal{U}_i(t)}_{j}(t) = w^{\mathcal{U}_i(t)}_{j}(t-1) - \eta \nabla F(w^{\mathcal{U}_i(t)}_{j}(t))$
%  }
%  }
%  $w^{\mathcal{U}_i(t)}(t) = \frac{\sum_{j=1}^{U_i(t)}\sum_{t=\tau_s k_g +1}^{\tau_s (k_g+1)}D^{\mathcal{U}_i(t)}_{j}(t)w^{\mathcal{U}_i(t)}_{j}(\tau_s (k_g)+1)}{\sum_{j=1}^{U_i(t)}\sum_{t=\tau_s k_g +1}^{\tau_s (k_g+1)}D^{\mathcal{U}_i(t)}_{j}(t)}$
%  }
%  \For{$\tilde{t} \in \{\tau_s (k_g+1)+1,\cdots, \tau_s (k_g+1) + t^p_i \} $}{
%  \For{$\mathcal{U}_i(t) \in \mathcal{U}$}{
%  Calculate Hessian-biased gradient descent
%  }
%  Send to access point for swarm wide average
%  }
%  $k_g += 1$
%  }
%  \For{Final time instances}{
%  \For{Every UAV swarm}{
%  Calculate Hessian-biased gradient descent
%  }
%  }
% \caption{Sequential FL-PFL}
% \end{algorithm}

==> old files/p1_v1.tex <==

\begin{proof} \label{sec:app_prop1}
We first apply the triangle inequality to extract the summation terms. The resulting expression is difficult to analyze directly due to the hierarchical nature of $\mathbf{w}_{k_2}(t)$, in which worker UAV to swarm leader relationships are embedded. Instead, we express the expected parameters within some global aggregation instance, i.e., $\mathbf{w}_{k_2}(t)$, as the expected parameters within some swarm-local aggregation instance, i.e., $\mathbf{w}_{k_1}(t)$ as follows:
\begin{equation}\label{eq:l1_p1}
\begin{aligned}
& \mathbb{E} \bigg[ \bigg\Vert \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t)  (\mathbf{w}_{k_2}^i(t) - \mathbf{w}_{k_2}(t)) \bigg\Vert \bigg]  \leq 
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) \mathbb{E} [\Vert \mathbf{w}_{k_2}^i(t) - \mathbf{w}_{k_2}(t) \Vert ] \\
& \equiv 
\tau_2^{-1} \hspace{-0.1in} \sum_{k_1=k_1^{\mathsf{start}}}^{\tau_2 k_2} \hspace{-0.1in}
\tau_1^{-1} \sum_{t= t_{k_1}^{\mathsf{start}}}^{\tau_1 k_1}
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t)   \mathbb{E} [\Vert \mathbf{w}_{k_1}^i(t) -  \mathbf{w}_{k_1}(t)\Vert],
\end{aligned}
\end{equation}
where $\Delta_u(t) = \sum_{i \in \mathcal{W}_u(t)}\Delta_i(t)$, $k_1^{\mathsf{start}} =  \tau_2(k_2-1)+1$, and $t_{k_1}^{\mathsf{start}} = \tau_1(k_1-1)+1$. Next, we recall the definition of $\mathbf{w}^{i}(t)$ from~\eqref{eq:meta_gradient_update}, and thus obtain (with the summations omitted for clarity):
\begin{equation}
\label{eq:l1_p2}
\begin{aligned}
&\mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t) - \mathbf{w}_{k_1}(t) \Vert] = \mathbb{E}\bigg[ \bigg\Vert \mathbf{w}_{k_1}^{i}(t) - \eta_2 \widetilde{\nabla F_i}(\mathbf{w}_{k_1}^{i}(t-1)) - \mathbf{w}_{k_1}(t-1) + \eta_2 \frac{1}{U}\sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}_{k_1}^{\hat{i}}(t-1)) \bigg\Vert \bigg] \\
&\leq \mathbb{E} [\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert] + \eta_2 \mathbb{E}\bigg[ \bigg\Vert \widetilde{\nabla F_i}(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{\hat{u} = 1}^{U}\frac{1}{\Delta_{\hat{u}}(t)} \sum_{i = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \widetilde{\nabla F_{\hat{i}}} (\mathbf{w}_{k_1}^{\hat{i}}(t-1) \bigg\Vert \bigg].
\end{aligned}
\end{equation}
% For simplicity of analysis, we define:
% \begin{equation}
% \begin{aligned}
% \xi_i(t) \triangleq \mathbb{E} \bigg[\Vert \mathbf{w}_{k_1}^{i}(t) -  \mathbf{w}_{k_1}(t) \Vert\bigg],
% \end{aligned}
% \end{equation}
% Then applying the update procedure \henry{on the right hand side of the prev eqn} for $\mathbf{w}_{k_1}^{i}$ gives: \henry{just write down epsilon i t is less than thing}
% \begin{equation}
% \begin{aligned}
% &\mathbb{E}\bigg[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert\bigg] + \beta \mathbb{E}\bigg[\Vert \widetilde{\nabla}F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{\hat{u} \in \mathcal{U}}\frac{1}{W_{\hat{u}}} \sum_{i\in \mathcal{W}_{\hat{u}}} \widetilde{\nabla}F_i(\mathbf{w}_{k_1}^{i}(t-1) \Vert\bigg] \\
% &= \xi_i(t-1) + \beta \mathbb{E}\bigg[\Vert \widetilde{\nabla}F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{\hat{u} \in \mathcal{U}}\frac{1}{W_{\hat{u}}} \sum_{i\in \mathcal{W}_{\hat{u}}} \widetilde{\nabla}F_i(\mathbf{w}_{k_1}^{i}(t-1) \Vert\bigg],
% \end{aligned}
% \end{equation}
Next, we move the $\mathbf{w}_{k_1}$ terms to the left hand side (LHS), and concisely re-format~\eqref{eq:l1_p2} in order to apply the result of Lemma~\ref{theory:lemma_sigma}.
{\small
\begin{equation}
\label{eq:l1_p3}
\begin{aligned}
&\mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t) - \mathbf{w}_{k_1}(t) \Vert] - \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert]
\leq 
\eta_2 \mathbb{E}\bigg[ \bigg\Vert \widetilde{\nabla F_i}(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{i = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \widetilde{\nabla F_{\hat{i}}} (\mathbf{w}_{k_1}^{\hat{i}}(t-1) \bigg\Vert \bigg] \\
% &= \beta \mathbb{E}\bigg[ \widetilde{\nabla}F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U}\sum_{\hat{u} \in \mathcal{U}}\frac{1}{W_{\hat{u}}}\sum_{i \in \mathcal{W}_{\hat{u}}} \widetilde{\nabla}F_i(\mathbf{w}_{k_1}^{i}(t-1)) \\
% &- \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) + \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) + \frac{1}{U} \sum_{\hat{u}\in \mathcal{U}} \frac{1}{W_{\hat{u}}} \sum_{i \in \mathcal{W}_{\hat{u}}} \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{\hat{u}\in \mathcal{U}} \frac{1}{W_{\hat{u}}} \sum_{i \in \mathcal{W}_{\hat{u}}} \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) \Vert \bigg] \\
&\leq \eta_2 \mathbb{E}[\Vert \widetilde{\nabla F_i}(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) \Vert ] 
+ \eta_2 \mathbb{E}\bigg[ \bigg\Vert \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \bigg( \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}_{k_1}^{\hat{i}}(t-1)) - \nabla F_{\hat{i}}(\mathbf{w}_{k_1}^{\hat{i}}(t-1)) \bigg) \bigg\Vert \bigg] \\
&+ \eta_2 \mathbb{E}\bigg[ \bigg\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \nabla F_{\hat{i}}(\mathbf{w}_{k_1}^{\hat{i}}(t-1)) \bigg\Vert \bigg].
\end{aligned}
\end{equation}
}
The first two terms on the right hand side (RHS) of~\eqref{eq:l1_p3} are now in the format of Lemma~\ref{theory:lemma_sigma}, with the second term needing the application of triangle inequality to extract the summations. We thus obtain:
\begin{equation} \label{eq:l1_p4}
\begin{aligned}
&\mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t) - \mathbf{w}_{k_1}(t) \Vert] - \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert]
\leq 
\eta_2 \bigg( \sigma_{F}^{i} + \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \sigma_{F}^{\hat{i}} \bigg) \\
&+ \eta_2 \mathbb{E}\bigg[ \bigg\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \nabla F_{\hat{i}}(\mathbf{w}_{k_1}^{\hat{i}}(t-1)) \bigg\Vert \bigg].
\end{aligned}
\end{equation}
The last term in~\eqref{eq:l1_p4} resembles that of Lemma~\ref{theory:lemma_gamma}, so we re-arrange~\eqref{eq:l1_p4} and thereby obtain:
\begin{equation}
\label{eq:l1_p5}
\begin{aligned}
&\mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t) - \mathbf{w}_{k_1}(t) \Vert] - \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert]
\leq 
\eta_2 \bigg( \sigma_{F}^{i} + \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \sigma_{F}^{\hat{i}} \bigg) \\
&+ \eta_2 \mathbb{E}\bigg[ \bigg\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1))
+ \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \bigg(\nabla F_{\hat{i}}(\mathbf{w}_{k_1}^{\hat{i}}(t-1)) - \nabla F_{\hat{i}}(\mathbf{w}_{k_1}(t-1)) \bigg) \bigg\Vert \bigg] \\
& + \eta_2 \mathbb{E}\bigg[ \bigg\Vert \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \nabla F_{\hat{i}}(\mathbf{w}_{k_1}(t-1)) \bigg\Vert \bigg].
\end{aligned}
\end{equation}
The last two terms in~\eqref{eq:l1_p5} resemble $\mu_F$-smooth condition and Lemma~\ref{theory:lemma_gamma}, respectively. Prior to applying those two results, we first apply the triangle inequality to move the summations, resulting in:
\begin{equation}
\label{eq:l1_p6}
\begin{aligned}
&\mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t) - \mathbf{w}_{k_1}(t) \Vert] - \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert]
\leq 
\eta_2 \bigg( \sigma_{F}^{i} + \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \sigma_{F}^{\hat{i}} \bigg) \\
&+ \eta_2 \mathbb{E} [ \Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert ]
+ \eta_2 \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \mathbb{E} [ \Vert \nabla F_{\hat{i}}(\mathbf{w}_{k_1}^{\hat{i}}(t-1)) - \nabla F_{\hat{i}}(\mathbf{w}_{k_1}(t-1)) \Vert ] \\
&+ \eta_2 \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \mathbb{E} [ \Vert \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \nabla F_{\hat{i}}(\mathbf{w}_{k_1}(t-1)) \Vert ].
\end{aligned}
\end{equation}
We now apply the $\mu_F$-smooth condition on the penultimate term in~\eqref{eq:l1_p6} and Lemma~\ref{theory:lemma_gamma} onto the final term in~\eqref{eq:l1_p6}, producing:
\begin{equation}
\label{eq:l1_p7}
\begin{aligned}
&\mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t) - \mathbf{w}_{k_1}(t) \Vert] - \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert]
\leq 
\eta_2 \bigg( \sigma_{F}^{i} + \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \sigma_{F}^{\hat{i}} \bigg) \\
&+ \eta_2 \mu_F \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert]
+ \eta_2 \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \mu_F \mathbb{E}[\Vert \mathbf{w}_{k_1}^{\hat{i}}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert] 
+ \eta_2 \frac{1}{U} \sum_{\hat{u} = 1}^{U} \gamma_F^{\hat{u}}.
\end{aligned}
\end{equation}
Recalling the omitted outer summations from~\eqref{eq:l1_p1} onto~\eqref{eq:l1_p7}, we see that there are redundant summations for those terms with $\hat{i}$ and $\hat{u}$ indexing. Therefore, we combine the RHS expressions for $\mathbb{E}[\Vert \mathbf{w}^{i}_{k_1}(t) - \mathbf{w}_{k_1}(t)\Vert]$, and obtain:
\begin{equation}
\label{eq:l1_p8}
\begin{aligned}
& \tau_2^{-1} \hspace{-0.1in} \sum_{k_1=k_1^{\mathsf{start}}}^{\tau_2 k_2} \hspace{-0.1in}
\tau_1^{-1} \sum_{t= t_{k_1}^{\mathsf{start}}}^{\tau_1 k_1}
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) 
\bigg( \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t) - \mathbf{w}_{k_1}(t) \Vert] - \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert] \bigg) \\
& \leq 
\tau_2^{-1} \hspace{-0.1in} \sum_{k_1=k_1^{\mathsf{start}}}^{\tau_2 k_2} \hspace{-0.1in}
\tau_1^{-1} \sum_{t= t_{k_1}^{\mathsf{start}}}^{\tau_1 k_1}
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) 
\eta_2 \bigg( \sigma_{F}^{i} + \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \sigma_{F}^{\hat{i}} + \frac{1}{U} \sum_{\hat{u}=1}^{U} \gamma_F^{\hat{u}} \bigg) \\
& + \tau_2^{-1} \hspace{-0.1in} \sum_{k_1=k_1^{\mathsf{start}}}^{\tau_2 k_2} \hspace{-0.1in}
\tau_1^{-1} \sum_{t= t_{k_1}^{\mathsf{start}}}^{\tau_1 k_1}
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) 
\eta_2 \mu_F \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert] \\
& + \tau_2^{-1} \hspace{-0.1in} \sum_{k_1=k_1^{\mathsf{start}}}^{\tau_2 k_2} \hspace{-0.1in}
\tau_1^{-1} \sum_{t= t_{k_1}^{\mathsf{start}}}^{\tau_1 k_1}
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t)
\eta_2 \frac{1}{U} \sum_{\hat{u} = 1}^{U} \frac{1}{\Delta_{\hat{u}}(t)} \sum_{\hat{i} = 1}^{W_{\hat{u}}(t)} \Delta_{\hat{i}}(t) \mu_F \mathbb{E}[\Vert \mathbf{w}_{k_1}^{\hat{i}}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert],
\end{aligned}
\end{equation}
which upon elimination of redundant summations yields:
\begin{equation}
\label{eq:l1_p9}
\begin{aligned}
& \tau_2^{-1} \hspace{-0.1in} \sum_{k_1=k_1^{\mathsf{start}}}^{\tau_2 k_2} \hspace{-0.1in}
\tau_1^{-1} \sum_{t= t_{k_1}^{\mathsf{start}}}^{\tau_1 k_1}
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) 
\bigg( \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t) - \mathbf{w}_{k_1}(t) \Vert] - \mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert] \bigg) \\
& \leq 
2 \eta_2 
\tau_2^{-1} \hspace{-0.1in} \sum_{k_1=k_1^{\mathsf{start}}}^{\tau_2 k_2} \hspace{-0.1in}
\tau_1^{-1} \sum_{t= t_{k_1}^{\mathsf{start}}}^{\tau_1 k_1}
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) 
\sigma_{F}^{i} 
+ 
\eta_2 
\tau_2^{-1} \hspace{-0.1in} \sum_{k_1=k_1^{\mathsf{start}}}^{\tau_2 k_2} \hspace{-0.1in}
\tau_1^{-1} \sum_{t= t_{k_1}^{\mathsf{start}}}^{\tau_1 k_1}
\frac{1}{U} \sum_{u=1}^{U} \gamma_F^{u} \\
& + 2 \eta_2 \mu_F \tau_2^{-1} \hspace{-0.1in} \sum_{k_1=k_1^{\mathsf{start}}}^{\tau_2 k_2} \hspace{-0.1in}
\tau_1^{-1} \sum_{t= t_{k_1}^{\mathsf{start}}}^{\tau_1 k_1}
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) 
\mathbb{E}[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert].
\end{aligned}
\end{equation}

The form of~\eqref{eq:l1_p9} suggests that a recursive approach would produce an expression for $\mathbb{E}[\Vert \mathbf{w}^{i}_{k_1}(t) - \mathbf{w}_{k_1}(t)\Vert]$ for some $k_1$-th local aggregation. However, for $t \in \{t_{k_1}^{\mathsf{start}},\cdots, \tau_1 k_1\}$, the initial worker $i$ parameters $\mathbf{w}_{k_1}^{i}(t_{k_1}^{\mathsf{start}})$ compared to the global average $\mathbf{w}_{k_1}(t_{k_1}^{\mathsf{start}})$ is not always $0$, especially if $\tau_2 \neq 1$. Instead of naively applying recursion, we revert to global aggregation steps $k_2$, and thus obtain:
\begin{equation}
\label{eq:l1_p10}
\begin{aligned}
& \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) 
\mathbb{E}[\Vert \mathbf{w}_{k_2}^{i}(t) - \mathbf{w}_{k_2}(t) \Vert] 
\leq 
\eta_2 
\frac{1}{U} \sum_{u=1}^{U} \bigg(  \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} 2\Delta_i(t) \sigma_{F}^{i} + \gamma_F^{u}\bigg) \\
& +
(1+ 2 \eta_2 \mu_F)
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) 
\mathbb{E}[\Vert \mathbf{w}_{k_2}^{i}(t-1) - \mathbf{w}_{k_2}(t-1) \Vert].
\end{aligned}
\end{equation}
The form of~\eqref{eq:l1_p10} allows us to apply recursion within some $k_2$ aggregation instance, i.e., for $t \in \{t_{k_2}^{\mathsf{start}},\cdots, \tau_1 \tau_2 k_2 \}$, where $t_{k_2}^{\mathsf{start}} \triangleq \tau_1(k_1^{\mathsf{start}}-1)+1$. And, since $\mathbf{w}^{i}_{k_2}(t_{k_2}^{\mathsf{start}}) = \mathbf{w}_{k_2}(t_{k_2}^{\mathsf{start}})$ due to the re-synchronization step of HN-PFL, we arrive at:
\begin{equation}
\label{eq:l1_p11}
\begin{aligned}
& \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) 
\mathbb{E}[\Vert \mathbf{w}_{k_2}^{i}(t) - \mathbf{w}_{k_2}(t) \Vert] 
\leq 
\eta_2 
\frac{1}{U} \sum_{u=1}^{U} \bigg(  \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} 2\Delta_i(t) \sigma_{F}^{i} + \gamma_F^{u}\bigg) \bigg[ \sum_{y=0}^{t- t_{k_2}^{\mathsf{start}}} (1+2\eta_2\mu_F)^y \bigg].
\end{aligned}
\end{equation}
Finally, realizing that the last term in~\eqref{eq:l1_p11} is the sum of finite geometric series, we obtain:
\begin{equation}
\label{eq:l1_p12}
\begin{aligned}
& \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} \Delta_i(t) 
\mathbb{E}[\Vert \mathbf{w}_{k_2}^{i}(t) - \mathbf{w}_{k_2}(t) \Vert] 
\leq 
\eta_2 
\frac{1}{U} \sum_{u=1}^{U} \bigg(  \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} 2\Delta_i(t) \sigma_{F}^{i} + \gamma_F^{u}\bigg) \frac{1-(1+2\eta_2\mu_F)^{t-t_{k_2}^{\mathsf{start}}+1}}{1 - (1+2\eta_2\mu_f)} \\
& 
=
\eta_2 
\frac{1}{U} \sum_{u=1}^{U} \bigg(  \frac{1}{\Delta_u(t)} \sum_{i=1}^{W_u(t)} 2\Delta_i(t) \sigma_{F}^{i} + \gamma_F^{u}\bigg) \frac{1-(1+2\eta_2\mu_F)^{t - \tau_1\tau_2 k_2 + \tau_1 \tau_2}}{1 - (1+2\eta_2\mu_f)} 
\end{aligned}
\end{equation}
% Separating the analysis of the last two terms in the above equation, we define:
% \begin{equation}
% \begin{aligned}
% & (i) \triangleq \beta \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) + \frac{1}{U} \sum_{\hat{u}\in \mathcal{U}} \frac{1}{W_{\hat{u}}} \sum_{i \in \mathcal{W}_{\hat{u}}} \bigg(\nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) \bigg)\Vert \bigg] \\
% & (ii) \triangleq \beta \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{U} \sum_{\hat{u}\in \mathcal{U}} \frac{1}{W_{\hat{u}}} \sum_{i \in \mathcal{W}_{\hat{u}}} \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert \bigg]. 
% \end{aligned}
% \end{equation}
% The analysis for $(i)$ requires moving the summations in~\eqref{eq:l1_p1}, so for continuity, we first analyze $(ii)$:
% \begin{equation}
% \begin{aligned}
% & \beta \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{U} \sum_{\hat{u}\in \mathcal{U}} \frac{1}{W_{\hat{u}}} \sum_{i \in \mathcal{W}_{\hat{u}}} \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert \bigg] \\
% &= \beta \mathbb{E}\bigg[\Vert \frac{1}{U} \sum_{\hat{u} \in \mathcal{U}} \bigg(\nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{W_{\hat{u}}} \sum_{i \in \mathcal{W}_{\hat{u}}} \nabla F_i(\mathbf{w}_{k_1}(t-1)) \bigg)  \Vert \bigg] \\
% &\leq \beta \frac{1}{U} \sum_{\hat{u} \in U} \mathbb{E} \bigg[ \Vert \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{W_{\hat{u}}} \sum_{i \in \mathcal{W}_{\hat{u}}} \nabla F_i(\mathbf{w}_{k_1}(t-1))\Vert \bigg] \leq \beta \frac{1}{U} \sum_{\hat{u} \in U} \gamma_{F}^{\hat{u}}.
% \end{aligned}
% \end{equation}

% In order to analyze $(i)$, we rearrange the sequence of summations in~\eqref{eq:l1_p1}:
% \begin{equation}
% \begin{aligned}
% &\frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \frac{1}{\tau_2}\sum_{k_1=\tau_2(k_2-1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t=\tau_1(k_1-1)+1}^{\tau_1 k_1} \mathbb{E} \Bigg[\Vert \mathbf{w}_{k_1}^i(t) -  \mathbf{w}_{k_1}(t)\Vert\Bigg] \equiv \\
% & \frac{1}{\tau_2}\sum_{k_1=\tau_2(k_2-1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t=\tau_1(k_1-1)+1}^{\tau_1 k_1} \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \mathbb{E} \Bigg[\Vert \mathbf{w}_{k_1}^i(t) -  \mathbf{w}_{k_1}(t)\Vert\Bigg]. 
% \end{aligned}
% \end{equation}

% Moving the inner two summations into (i), thereafter applying the Lipschitz smooth property of the loss functions, and noting that the average of an average remains Lipschitz smooth gives:
% \begin{equation}
% \begin{aligned}
% & \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \beta \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) + \frac{1}{U} \sum_{\hat{u}\in \mathcal{U}} \frac{1}{W_{\hat{u}}} \sum_{i \in \mathcal{W}_{\hat{u}}} \bigg(\nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) \bigg)\Vert \bigg] \\
% & \leq \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \beta \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert \bigg] \\
% &+ \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \beta \mathbb{E} \bigg[\Vert \frac{1}{U} \sum_{\hat{u}\in \mathcal{U}} \frac{1}{W_{\hat{u}}} \sum_{i \in \mathcal{W}_{\hat{u}}} \bigg(\nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) \bigg)\Vert \bigg] \\
% & \leq \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \beta \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert \bigg] \\
% &+ \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u}\frac{1}{U} \sum_{\hat{u}\in \mathcal{U}}  \frac{1}{W_{\hat{u}}} \sum_{i \in \mathcal{W}_{\hat{u}}} \beta \mathbb{E} \bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert \bigg] \\
% & \leq \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} 2\beta L_{F} \xi_i(t-1).
% \end{aligned}
% \end{equation}

% Now, combining (i), (ii), and~\eqref{eq:l1_p_xi_diff} with the swapped summation sequence: 
% \begin{equation}
% \begin{aligned}
% & \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \bigg( \xi_i(t) - \xi_i(t-1) \bigg) \\ 
% & \leq \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u}  \beta (\sigma_{F}^{u} + \frac{1}{U}\sum_{\hat{u} \in \mathcal{U}} \sigma_{F}^{\hat{u}}) + \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} 2\beta L_{F} \xi_i(t-1) + \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \beta \frac{1}{U} \sum_{\hat{u} \in U} \gamma_{F}^{\hat{u}}.
% \end{aligned}
% \end{equation}

% Rearranging gives:
% \begin{equation}
% \begin{aligned}
% & \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \xi_i(t) \\
% & \leq \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u}  \beta (\sigma_{F}^{u} + \frac{1}{U}\sum_{\hat{u} \in \mathcal{U}} \sigma_{F}^{\hat{u}}) + \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \bigg(1+2\beta L_{F}\bigg) \xi_i(t-1) + \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \beta \frac{1}{U} \sum_{\hat{u} \in U} \gamma_{F}^{\hat{u}}.
% \end{aligned}
% \end{equation}

% Noting that the inner summation is over time $t \in [\tau_1 (k_1-1)+1,\cdots,\tau_1 k_1]$, we solve the above recursively over this time interval while dropping the summation over $u$ and $i$ for simplicity, giving:
% \begin{equation}
% \begin{aligned}
% &\xi_i(t) \leq {\bigg(1+2\beta L_F \bigg)}^{t-(\tau_1 k_1)} + \beta \bigg(\sigma_{F}^{u} + \frac{1}{U}\sum_{\hat{u} \in \mathcal{U}} (\sigma_{F}^{\hat{u}} + \gamma_{F}^{\hat{u}}) \bigg) \sum_{y = 0}^{t-(\tau_1 k_1)} (1+2\beta L_F)^{y} \\
% &= {\bigg(1+2\beta L_F \bigg)}^{t-(\tau_1 k_1)} + \beta \bigg(\sigma_{F}^{u} + \frac{1}{U}\sum_{\hat{u} \in \mathcal{U}} (\sigma_{F}^{\hat{u}} + \gamma_{F}^{\hat{u}}) \bigg) \frac{1-(1+2\beta L_F)^{t-(\tau_1 k_1)}}{1-(1+2\beta L_F)}.
% \end{aligned}
% \end{equation}

% Finally, rearranging into the form in~\eqref{eq:l1_p1}, by reverting $\xi_i(t)$ produces:

% \begin{equation}
% \begin{aligned}
% & \frac{1}{\tau_2}\sum_{k_1=\tau_2(k_2-1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t=\tau_1(k_1-1)+1}^{\tau_1 k_1} \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \mathbb{E} \Bigg[\Vert \mathbf{w}_{k_1}^i(t) -  \mathbf{w}_{k_1}(t)\Vert\Bigg] \\ 
% &\leq \frac{1}{\tau_2}\sum_{k_1=\tau_2(k_2-1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t=\tau_1(k_1-1)+1}^{\tau_1 k_1} \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i=1}^{W_u} \Bigg[ {\bigg(1+2\beta L_F \bigg)}^{t-(\tau_1 k_1)} \\
% &+ \beta \bigg(\sigma_{F}^{u} + \frac{1}{U}\sum_{\hat{u} \in \mathcal{U}} (\sigma_{F}^{\hat{u}} + \gamma_{F}^{\hat{u}}) \bigg) \frac{1-(1+2\beta L_F)^{t-(\tau_1 k_1)}}{1-(1+2\beta L_F)} \Bigg].
% \end{aligned}
% \end{equation}

\end{proof}

==> old files/p1_v2.tex <==

\begin{proof} \label{sec:app_prop1} 
To bound
\begin{equation} \label{eq:prop1_eq1}
\begin{aligned}
&\mathbb{E}\bigg[ \bigg\Vert \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u}  \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\bigg(\mathbf{w}^{i}(\tau_1 \tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2)
\bigg) \bigg\Vert \bigg],
\end{aligned}
\end{equation}
where $\Delta_i(k_2) = \sum_{t = \tau_1 \tau_2 k_2 - \tau_1}^{\tau_1 \tau_2 k_2} \Delta_i(t)$, 
and $\Delta_u(k_2) = \sum_{i=1}^{W_u} \Delta_i(k_2)$, we 
% The hierarchical relationships between $\mathbf{w}^i$ and $\mathbf{w}$ are unclear in~\eqref{eq:prop1_eq1}. 
introduce $\mathbf{w}^{u}(\tau_1\tau_2k_2)$, which yields:
% to separate the expression into two separate relationships, mimicking the two-layer aggregation system of our problem:
\begin{equation} \label{eq:prop1_eq2}
\begin{aligned}
&\mathbb{E}\bigg[ \bigg\Vert 
\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\bigg(\mathbf{w}^{i}(\tau_1 \tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) + \mathbf{w}^{u}(\tau_1 \tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2)
\bigg) 
\bigg\Vert \bigg] \\
&\leq 
\underbrace{\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E}[\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1\tau_2 k_2) \Vert ]  }_{(i)}
+ 
\underbrace{
\frac{1}{U}\sum_{u = 1}^{U}
\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1\tau_2 k_2)
\Vert]}_{(ii)}.
\end{aligned}
\end{equation} 

\noindent
% The analysis of the two terms in~\eqref{eq:prop1_eq2} requires different techniques and so we perform their analyses separately. 
% First, we upper bound $\mathbf{w}^{i}(\tau_1 \tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2)$ by recalling the meta-gradient update procedure at worker UAV $i$ and the local aggregation expression for $\mathbf{w}^{u}$, i.e., $\mathbf{w}^{u} (\tau_1 \tau_2 k_2) = \frac{1}{\Delta_u(k_2)}\sum_{i=1}^{W_u} \Delta_i(k_2) \mathbf{w}^{i} (\tau_1 \tau_2 k_2)$. 
% Thus, omitting the outer summations, we obtain:
We first upper bound~\eqref{eq:prop1_eq2}(i), omitting the summations for simplicity:
\begin{equation} \label{eq:prop1_eq3}
\begin{aligned} 
& \mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) \Vert ]
\overset{(a)}{=} \mathbb{E} \bigg[ \bigg\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_u(k_2)} \mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2) \bigg\Vert \bigg] \\
& \overset{(b)}{=} \mathbb{E} \bigg[ \bigg\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2-1) - \eta_2 \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1))
- \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}} (k_2) }{\Delta_u(k_2)} 
\bigg(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1) - \eta_2 \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg)
\bigg\Vert \bigg] \\
% \end{aligned}
% \end{equation}
% \noindent
% Already, we can see there exists a recursive relationship between $\mathbf{w}^{i}(\tau_1 \tau_2 k_2)$ and $\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)$. The relationship between the mini-batch meta-gradients is less clear however. To progress, we then compare the mini-batch meta-gradients $\widetilde{\nabla F_i}$ and $\widetilde{\nabla F_u} =  \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}$ with respect to the true gradients $\nabla F_i$ and $\nabla F_u = \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \nabla F_i$. Thus:
% \begin{equation} \label{eq:prop1_eq4}
% \begin{aligned}
% &\mathbb{E} \bigg[ \bigg\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2-1) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1))
% - \frac{1}{\Delta_u(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) 
% \bigg(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1) -\widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg) 
% \bigg\Vert \bigg] \\
& \overset{(c)}{\leq} 
\underbrace{\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert ]}_{(i)}
+ 
\underbrace{\eta_2 
\mathbb{E} [ \Vert 
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) 
\Vert ]}_{(ii)} \\
& + 
\underbrace{\eta_2 
\mathbb{E} \bigg[ \bigg\Vert 
\sum_{\hat{i}=1}^{W_u} \frac{\Delta_{\hat{i}}(k_2) }{\Delta_u(k_2)} \bigg( \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) - \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg) 
\bigg\Vert \bigg]}_{(iii)} \\
&+
\underbrace{\eta_2 
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2) }{\Delta_{u}(k_2)} \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert \bigg]}_{(iv)},
\end{aligned}
\end{equation}
where $(a)$ is the aggregation rule of $\mathbf{w}^u$, $(b)$ uses the gradient update from~\eqref{eq:meta_gradient_update}, and $(c)$ introduces $\nabla F_i$ and $\nabla F_u$ terms before applying triangle inequality. 
The bounds for~\eqref{eq:prop1_eq3}(ii) and~\eqref{eq:prop1_eq3}(iii) follow immediately from Lemma~\ref{theory:lemma_sigma}, and we analyze~\eqref{eq:prop1_eq3}(iv), while recalling the summations from~\eqref{eq:prop1_eq2} as follows:
% We use Lemma~\ref{theory:lemma_sigma} to bound~\eqref{prop1_eq3}(ii) and~\eqref{prop1_eq3}(iii). 
% \noindent
% The $\mathbb{E}[\Vert \nabla F_i - \widetilde{\nabla F_i} \Vert]$ terms are easy to upper bound via Lemma~\ref{theory:lemma_sigma}. However, the final term in~\eqref{eq:prop1_eq4} poses two challenges: (i) the loss function gradients $\nabla F_i$ are on different datasets - hence entirely different loss functions, and (ii) the parameters $\mathbf{w}^{i}$ are unique for each worker UAV $i \in \mathcal{W}_u$. We address these two challenges in tandem by introducing $\nabla F_i(\mathbf{w}^u)$ and $\nabla F_{\hat{i}}(\mathbf{w}^u)$, which allows us to take advantage of the $\mu_F$-Lipschitz smooth property determined earlier in the main text.
% For simplicity, we will first analyze the last term in~\eqref{eq:prop1_eq4} in isolation and then recombine its result with that of~\eqref{eq:prop1_eq4}.
\begin{align} \label{eq:prop1_eq4}
% \begin{aligned}
& \eta_2 
\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)}  \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert \bigg] \\ \nonumber
%%%%        (a)
& \overset{(a)}{=}
\eta_2 
\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
+ \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
\\ \nonumber
& 
- \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)} 
\bigg( 
\nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1)) 
+ \nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
- \nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg)
\bigg\Vert \bigg] \\ \nonumber
% \end{aligned}
% \end{equation}
% \begin{equation} \label{eq:prop1_eq6}
% \begin{aligned}
%%%     (b)
& \overset{(b)}{\leq} 
\eta_2\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
\Vert ]
\\ \nonumber
& + \eta_2
\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} \bigg[ \bigg\Vert  \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)}
\bigg(
\nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
- \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1)) 
\bigg)
\bigg\Vert \bigg] \\ \nonumber
& + \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\mathbb{E} \bigg[ \bigg\Vert \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2) }{\Delta_{u}(k_2)} 
\nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg \Vert \bigg] \\ \nonumber
%%%       (c)
& \overset{(c)}{\leq} 
\eta_2\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
\Vert ]
\\ \nonumber
& + 
\eta_2
\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)}
\mathbb{E} \bigg[ \bigg\Vert 
\nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
- \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1)) 
\bigg\Vert \bigg]
\\ \nonumber
& 
+ \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\mathbb{E} \bigg[ \bigg\Vert \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_{u}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg \Vert \bigg] \\ \nonumber
%%%       (d)
& \overset{(d)}{\leq} 
\eta_2 \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} \mu_F 
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 -1) \Vert]
\\ \nonumber
& +
\eta_2
\frac{1}{U}\sum_{u = 1}^{U} %\sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)}
\mu_F 
\mathbb{E} [ \Vert \mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1) - \mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2 -1) \Vert ] 
\\ \nonumber
& 
+ \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\mathbb{E} \bigg[ \bigg\Vert \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_{u}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg \Vert \bigg]  \\ \nonumber
%%%       (e)
& \overset{(e)}{\leq} 
2 \mu_F \eta_2 \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 -1) \Vert]
+
\eta_2 \frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u},
\end{align}
% \end{equation}
where (a) introduces $\nabla F_i(\mathbf{w}^u)$ and $\nabla F_{\hat{i}}(\mathbf{w}^u)$,
(b) applies triangle inequality, 
(c) recalls the agggregation rule of $\nabla F_u$ and applies triangle inequality, 
(d) uses $\mu_F$-smoothness (i.e., $\Vert \nabla F_i(\mathbf{w}) - \nabla F_i (\mathbf{w}') \Vert \leq \mu_F \Vert \mathbf{w} - \mathbf{w}' \Vert$ $\forall i \in \cup_{u \in \mathcal{U}} \mathcal{W}_u$), 
and (e) leverages Lemma~\ref{theory:lemma_gamma}.
Combining~\eqref{eq:prop1_eq3} and~\eqref{eq:prop1_eq4} yields: 
%Now, we (a) combine the result of~\eqref{eq:prop1_eq4} into~\eqref{eq:prop1_eq3} with the summations returning, (b) apply triangle inequality and Lemma 1, and (c) use the result in~\eqref{eq:prop1_eq6}. Hence, we obtain:
\begingroup
\allowdisplaybreaks
%\begin{equation} 
\begin{align}
& \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) \Vert ] \label{eq:prop1_eq5} \\
%%%     (a)
& \overset{(a)}{\leq} 
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert ] \nonumber\\
& + \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert 
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) 
\Vert ] \nonumber\\
& + \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} \bigg[ \bigg\Vert 
\sum_{\hat{i}=1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_u(k_2)} \bigg( \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) - \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg) 
\bigg\Vert \bigg] \nonumber\\
&+ \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)} \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert \bigg] \nonumber\\
%%%         (b)
& \overset{(b)}{\leq}
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert ] 
+ 
2 \eta_2 \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\sigma_F^{i}(\tau_1\tau_2 k_2 -1)
\nonumber\\
& + \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2) }{\Delta_{u}(k_2)} \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert \bigg] \nonumber \\
%%%         (c)
& \overset{(c)}{\leq}
(1+ 2 \eta_2 \mu_F)
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert ] 
\nonumber\\
& + 2\eta_2  \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}  
\sigma_F^{i}(\tau_1 \tau_2 k_2 -1)
+
\eta_2
\frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u},
\nonumber
\end{align}
%\end{equation}
\endgroup
where $(a)$ restates~\eqref{eq:prop1_eq3} with the previously omitted summations, $(b)$ applies triangle inequality and Lemma~\ref{theory:lemma_sigma}, and $(c)$ uses the result in~\eqref{eq:prop1_eq4}. Solving~\eqref{eq:prop1_eq5} recursively yields:
% \noindent Comparing left and right hand sides of~\eqref{eq:prop1_eq7}, we see the recursive relationship between $\mathbb{E}[\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1\tau_2 k_2) \Vert]$ 
% and 
% $\mathbb{E}[\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2-1) - \mathbf{w}^{u}(\tau_1\tau_2 k_2-1) \Vert]$ emerge. 
% In our problem formulation, swarm aggregations at swarm $u$ occur among the swarm leader $z_u$ and its worker UAVs $i \in \mathcal{W}_u$ with period $\tau_1$. Therefore, $\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -\tau_1) = \mathbf{w}^{u}(\tau_1 \tau_2 k_2 - \tau_1)$. Performing the recursion on~\eqref{eq:prop1_eq7} for $\tau_1$ instances starting from $\tau_1 \tau_2 k_2$ thus yields:
\begin{align} \label{eq:prop1_eq6}
& \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2) }{\Delta_u(k_2)}  \mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) \Vert ] \\
& 
%%%%        (a)
\overset{(a)}{\leq }
% \bigg(2\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
% \sigma_F^{i} 
% +
% \frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u} \bigg)
% \sum_{t = 0}^{\tau_1 - 1} (1+ 2\mu_F)^t
2 \eta_2 \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u}  \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\bigg(
\sum_{y=0}^{\tau_1 -1}
\sigma_F^{i}(\tau_1 \tau_2 k_2 - 1 -y) (1+2\eta_2\mu_F)^{y}
\bigg)
+ \eta_2
\frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u}
\frac{1 - (1+2 \eta_2 \mu_F)^{\tau_1}}{1- (1+2\eta_2\mu_F)}\\
&
%%%%        (b)
\overset{(b)}{\leq}
\bigg(
2 \eta_2 \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u}  \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\sum_{y=0}^{\tau_1 -1}
\sigma_F^{i}(\tau_1 \tau_2 k_2 - 1 -y)
+
\eta_2 \frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u}
\bigg)
\frac{1 - (1+2 \eta_2 \mu_F)^{\tau_1}}{1- (1+2 \eta_2 \mu_F)},
\end{align}
where $(a)$ is the result of recursion and the finite sum of geometric series, and $(b)$ uses $\sum_i a_i b_i \leq \sum_i a_i \sum_i b_i$ $\forall a_i, b_i \geq 0$. 
% where the last inequality comes from , and the finite sum of geometric series.
Next, we bound~\eqref{eq:prop1_eq2}(ii) as follows:
%i.e., $\mathbb{E} [\Vert \mathbf{w}^{u}(\tau_1 \tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert]$. We begin by omitting the outer summations for clarity and expand the form of $\mathbf{w}$, which produces:
\begin{equation} \label{eq:prop1_eq7}
\begin{aligned}
& \mathbb{E} [ \Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert ] 
= \mathbb{E} \bigg[ \bigg\Vert  \mathbf{w}^{u}(\tau_1\tau_2 k_2)
- \frac{1}{U} \sum_{\hat{u}=1}^{U} 
\mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2) \bigg\Vert \bigg] \\
& =
\mathbb{E} \bigg[ \bigg\Vert  \mathbf{w}^{u}(\tau_1\tau_2 k_2-1)
- \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1))
- \frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2-1) 
- \widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
\bigg)
\bigg\Vert \bigg].
\end{aligned}
\end{equation}

\noindent 
Similarly to the analysis of $\mathbb{E}[\Vert \mathbf{w}^{i} - \mathbf{w}^{u} \Vert ]$ in~\eqref{eq:prop1_eq4}, we first compare the meta-gradients $\widetilde{\nabla F_u}$ against the true gradient $\nabla F_u$. Thus, starting from~\eqref{eq:prop1_eq9}, we (a) show an equivalent form and then (b) apply triangle inequality to simplify analysis:
\begin{equation} \label{eq:prop1_eq10}
\begin{aligned}
%%%         (a)
& \overset{(a)}{=}
\mathbb{E} \bigg[ \bigg\Vert  \mathbf{w}^{u}(\tau_1\tau_2 k_2-1)
- \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) 
+ \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
\\
&
- \frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2-1) 
- \widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
+ \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
\bigg)
\bigg\Vert \bigg] \\
%%%         (b)
& \overset{(b)}{\leq} 
\mathbb{E} \bigg[ \bigg\Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \frac{1}{U} \sum_{\hat{u} =1}^{U} \mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2 -1)
\bigg\Vert \bigg]
+
\mathbb{E} [ \Vert \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) \Vert ]\\
& + \mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)) 
\bigg)
\bigg\Vert \bigg] \\
& + \mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) \bigg\Vert \bigg].
\end{aligned}
\end{equation}

\noindent
The middle two terms on the right hand side of~\eqref{eq:prop1_eq10} are easily bounded once we expand the hierarchy and apply Lemma~\ref{theory:lemma_sigma}. As in~\eqref{eq:prop1_eq4}, the main challenge in~\eqref{eq:prop1_eq10} is the last term due to (i) the loss function gradients $\nabla F_u$ are on different datasets - hence entirely different loss functions, and (ii) the parameters $\mathbf{w}^{u}$ are unique for each swarm UAV $u \in \mathcal{U}$. We address these two challenges in tandem by introducing $\nabla F_u(\mathbf{w})$ and $\nabla F_{\hat{u}}(\mathbf{w})$, which allows us to take advantage of both $\mu_F$-Lipschitz smooth property and Lemma~\ref{theory:lemma_gamma}. Hence:
\begin{align} \label{eq:prop1_eq11}
& \mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
\bigg\Vert \bigg] \nonumber \\
& = 
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}(\tau_1\tau_2 k_2-1))
+ \nabla F_{\hat{u}} (\mathbf{w}(\tau_1\tau_2 k_2-1))
\bigg)
\nonumber \\
& 
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
+ \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\bigg\Vert \bigg].
\end{align}

\noindent
We now bound~\eqref{eq:prop1_eq10} which requires bringing back the previously omitted summations. Then, we 
(a) combine~\eqref{eq:prop1_eq10} and~\eqref{eq:prop1_eq11}, 
(b) expand the form of $\nabla F_{\hat{u}}$ into its constituent $\nabla F_{i}$ and apply triangle inequality,
(c) use Lemma~\ref{theory:lemma_sigma} and $\mu_F$-Lipschitz smooth,
and (d) expand the summations and use Lemma~\ref{theory:lemma_gamma}. For clarity, we explain from $\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert]$ as follows:
\begin{align} \label{eq:prop1_eq12}
& \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert] \nonumber\\
%%%     (a)
& \overset{(a)}{\leq}
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} \bigg[ \bigg\Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \frac{1}{U} \sum_{\hat{u} =1}^{U} \mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2 -1)
\bigg\Vert \bigg] 
\nonumber \\
& +
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [ \Vert \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) \Vert ] 
\nonumber \\
& + 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)) 
\bigg)
\bigg\Vert \bigg] 
\nonumber \\
& + 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}(\tau_1\tau_2 k_2-1))
+ \nabla F_{\hat{u}} (\mathbf{w}(\tau_1\tau_2 k_2-1))
\bigg)
\nonumber \\
& 
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
+ \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\bigg\Vert \bigg]
\nonumber \\
%%%         (b)
& \overset{(b)}{\leq} 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} \bigg[ \bigg\Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \frac{1}{U} \sum_{\hat{u} =1}^{U} \mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2 -1)
\bigg\Vert \bigg] 
\nonumber \\
& + 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{\Delta_u(k_2)} \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [ \Vert \nabla F_i (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \widetilde{\nabla F_i}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) \Vert ] 
\nonumber \\
& + 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \frac{1}{\Delta_{\hat{u}}(k_2)} \sum_{i = 1}^{W_{\hat{u}}} \Delta_i(k_2) 
\mathbb{E} [ \Vert
\widetilde{\nabla F_{i}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{i} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)) 
\Vert ] 
\nonumber \\
& + 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \frac{1}{\Delta_{\hat{u}}(k_2)} \sum_{i = 1}^{W_{\hat{u}}} \Delta_i(k_2) 
\mathbb{E} [ \Vert 
\nabla F_{i} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{i} (\mathbf{w}(\tau_1\tau_2 k_2-1))
\Vert ]
\nonumber \\
& + 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{\Delta_{u}(k_2)} \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [\Vert \nabla F_{i} (\mathbf{w}(\tau_1\tau_2 k_2-1))
- \nabla F_i (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
\Vert ] 
\nonumber \\
& + 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \nabla F_{\hat{u}} (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\bigg\Vert \bigg]
\nonumber \\
%%%         (c)
& \overset{(c)}{\leq} 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [ \Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}(\tau_1 \tau_2 k_2 -1)
\Vert ] 
\nonumber \\
& + 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{\Delta_u(k_2)} \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\sigma_F^i(\tau_1\tau_2 k_2 -1) \nonumber \\
& + 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \frac{1}{\Delta_{\hat{u}}(k_2)} \sum_{i = 1}^{W_{\hat{u}}} \Delta_i(k_2) 
\sigma_F^i(\tau_1 \tau_2 k_2 -1)
\nonumber \\
& + \mu_F 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \frac{1}{\Delta_{\hat{u}}(k_2)} \sum_{i = 1}^{W_{\hat{u}}} \Delta_i(k_2) 
\mathbb{E} [ \Vert 
\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)
- \mathbf{w}(\tau_1\tau_2 k_2-1)
\Vert ]
\nonumber \\
& + \mu_F 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{\Delta_{u}(k_2)} \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [\Vert \mathbf{w}(\tau_1\tau_2 k_2-1)
- \mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)
\Vert ] 
\nonumber \\
& + 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [\Vert 
\nabla F (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\Vert]
\nonumber \\
%%%         (d)
& \overset{(d)}{\leq} 
(1+ 2\mu_F) \frac{1}{U}\sum_{u = 1}^{U} \mathbb{E} [ \Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}(\tau_1 \tau_2 k_2 -1)
\Vert ]
+ 
2 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\sigma_F^i(\tau_1 \tau_2 k_2 -1)
+ \gamma_F.
\end{align}

\noindent 
Comparing left and right hand sides of~\eqref{eq:prop1_eq12}, we see the recursive relationship between $\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1\tau_2 k_2) \Vert]$ 
and 
$\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2-1) - \mathbf{w}(\tau_1\tau_2 k_2-1) \Vert]$ emerge. 
Differently from swarm aggregations, global aggregations among all swarm leaders $\{z_u\}$, $\forall u \in \mathcal{U}$ only occurs every $\tau_2$ swarm aggregations, i.e., every $\tau_1 \tau_2$ time instances. Therefore, $\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -\tau_1\tau_2) = \mathbf{w}(\tau_1 \tau_2 k_2 - \tau_1\tau_2)$. Performing the recursion on~\eqref{eq:prop1_eq12} for $\tau_1\tau_2$ instances starting from $\tau_1 \tau_2 k_2$ thus yields:
\begin{equation}
\label{eq:prop1_eq13}
\begin{aligned}
& \frac{1}{U}\sum_{u = 1}^{U} \mathbb{E} [ \Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert ] 
\\
& \leq 
2\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\bigg(
\sum_{y=0}^{\tau_1\tau_2-1}\sigma_F^{i}(\tau_1\tau_2 k_2-1-y) (1+2\mu_F)^{y}
\bigg)
+
\gamma_{F}
\frac{1 - (1+2 \mu_F)^{\tau_1 \tau_2}}{1- (1+2\mu_F)} \\
& \leq
\bigg(
2\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\sum_{y=0}^{\tau_1\tau_2-1}\sigma_F^{i}(\tau_1\tau_2 k_2-1-y)
+
\gamma_{F}
\bigg)
\frac{1 - (1+2 \mu_F)^{\tau_1 \tau_2}}{1- (1+2\mu_F)},
\end{aligned}
\end{equation}
where the last inequality comes from $\sum_{i} a_i b_i \leq \sum_{i} a_i \sum_{i} b_i$ $\forall a_i, b_i \geq 0$ followed by the sum of finite geometric series.
Finally, combining the results of~\eqref{eq:prop1_eq8} and~\eqref{eq:prop1_eq13} back into~\eqref{eq:prop1_eq2} and shifting the summation from $y=0$ to $y=1$ yields the result:
\begin{equation}
\label{eq:prop1_eq14}
\begin{aligned}
& \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\bigg( \mathbb{E}[\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1\tau_2 k_2) \Vert ] + \mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1\tau_2 k_2)
\Vert] \bigg) \\
& \leq 
\bigg(
2\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\sum_{y=1}^{\tau_1}
\sigma_F^{i}(\tau_1 \tau_2 k_2 - y)
+
\frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u}
\bigg)
\frac{1 - (1+2 \mu_F)^{\tau_1}}{1- (1+2\mu_F)}\\
& +
\bigg(
2\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\sum_{y=1}^{\tau_1\tau_2}\sigma_F^{i}(\tau_1\tau_2 k_2-y)
+
\gamma_{F}
\bigg)
\frac{1 - (1+2 \mu_F)^{\tau_1 \tau_2}}{1- (1+2\mu_F)}.
\end{aligned}
\end{equation}

\end{proof}

==> old files/p2_v1.tex <==

\begin{proof}
First, we simplify the expectation:
\begin{equation} \label{eq:l2_p1}
\begin{aligned}
&\mathbb{E}\bigg[\frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \Vert \mathbf{w}_{k_2}^{i}(t) - \mathbf{w}_{k_2}(t) \Vert^2\bigg] \\
&\leq \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \mathbb{E}\bigg[ \Vert \mathbf{w}_{k_2}^{i}(t) - \mathbf{w}_{k_2}(t) \Vert^2\bigg] \\
& = \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \frac{1}{\tau_2} \sum_{k_1 = \tau_2(k_2 - 1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t = \tau_1 (k_1 -1)+1}^{\tau_1 k_1} \mathbb{E}\bigg[ \Vert \mathbf{w}_{k_1}^{i}(t) - \mathbf{w}_{k_1}(t) \Vert^2\bigg]
\end{aligned}
\end{equation}

We first define:
\begin{equation}
\Upsilon_i(t) \triangleq \mathbb{E}\bigg[ \Vert \mathbf{w}_{k_1}^{i}(t) - \mathbf{w}_{k_1}(t) \Vert^2\bigg],
\end{equation}

and we can express $\Upsilon_i(t)$ as:

\begin{equation}
\begin{aligned}
\Upsilon_i(t) = \mathbb{E}\bigg[ \Vert \mathbf{w}_{k_1}^{i}(t-1) - \beta \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \bigg( \mathbf{w}_{k_1}^{i}(t-1) - \beta \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) \bigg) \Vert^2\bigg].
\end{aligned}
\end{equation}

We denote the following property as $(*)$ due  to its frequent use and note that it applies for all $\phi \in \mathbb{R}^{+}$:
\begin{equation} \label{eq:l2_astericks}
(*): \Vert a+b \Vert^2 \leq (1+\phi)\Vert a \Vert^2 + (1+\frac{1}{\phi})\Vert b \Vert^2.
\end{equation}

So, using $(*)$ on $\Upsilon_i(t)$:
\begin{equation} \label{eq:l2_proof_split}
\begin{aligned}
&\Upsilon_i(t) \leq (1+\phi) \mathbb{E}\bigg[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \mathbf{w}_{k_i}^{i}(t-1) \Vert^2\bigg] \\
&+ (1+\frac{1}{\phi}) \beta^2 \mathbb{E}\bigg[\Vert \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) \Vert^2\bigg] \\
&= (1+\phi) \Upsilon_i(t-1) + (1+\frac{1}{\phi}) \beta^2 \mathbb{E}\bigg[\Vert \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) \Vert^2\bigg].
\end{aligned}
\end{equation}

Focusing on the second equation in the previous inequality:
\begin{equation}
\begin{aligned}
&\mathbb{E}\bigg[\Vert \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) \Vert^2\bigg] 
= \mathbb{E}\bigg[\Vert \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) \\
&+ \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) + \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) \Vert^2\bigg] \\
&\leq 2 \mathbb{E}\bigg[\Vert \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1))
+
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \bigg(\widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1))\bigg) \Vert^2\bigg] \\
&+ 2\mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) \Vert^2\bigg],
\end{aligned}
\end{equation}
where the inequality comes from application of $(*)$ with $\phi = 1$.

For clarity, we define:
\begin{equation}
\begin{aligned}
&(a): 2 \mathbb{E}\bigg[\Vert \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1))
+
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \bigg(\widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1))\bigg) \Vert^2\bigg] \\
&(b): 2\mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) \Vert^2\bigg].
\end{aligned}
\end{equation}

We now focus on the analysis of $(a)$ using $(*)$ with $\phi =1$ and Cauchy-Schwarz inequality:
\begin{equation} \label{eq:l2_proof_eqn_a}
\begin{aligned}
&(a) \leq 4 \mathbb{E}\bigg[\Vert \widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) \Vert^2 \bigg]
+ 4 \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \mathbb{E} \bigg[ \Vert 
\widetilde{\nabla} F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) \Vert^2\bigg] \\
&\leq 4 {(\sigma_{F}^{u})}^2 + 4 \frac{1}{U} \sum_{u=1}^{U} {(\sigma_{F}^{u})}^2.
\end{aligned}
\end{equation}
Note that the final step uses Lemma 4.3 from~\cite{fallah2020personalized}.

Next, we analyze $(b)$, applying $(*)$ and then recalling the definition of $\eta_i(t)$ from the proof of the previous Lemma~\eqref{}:
\begin{equation} \label{eq:l2_proof_eqn_b}
\begin{aligned}
&(b) = 2\mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) + \nabla F(w_{k_1}(t-1)) -\nabla F(w_{k_1}(t-1)) \\ 
&+ \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}(t-1))\Vert^2\bigg] \\
&\leq 4 \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \bigg( \nabla F_i(\mathbf{w}_{k_1}^{i}(t-1)) - \nabla F_i(\mathbf{w}_{k_1}(t-1)) \bigg) \Vert^2\bigg]\\
& + 4 \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert^2\bigg] \\
& = 4 \mathbb{E}\bigg[\Vert \eta_i(t-1) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \eta_i(t-1) \Vert^2 \bigg] + 4 \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert^2\bigg].
\end{aligned}
\end{equation}

Before continuing, we separately analyze the second term in the above inequality:
\begin{equation}
\begin{aligned}
& 4 \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert^2\bigg] = 4 \mathbb{E}\bigg[\Vert \frac{1}{U}\sum_{u = 1}^{U} \nabla F_i(\mathbf{w}_{k_1}(t-1)) \\
&- \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert^2\bigg] 
\leq 4 \frac{1}{U} \sum_{u=1}^{U} \mathbb{E} \bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert^2\bigg] \leq 4 \frac{1}{U} \sum_{u=1}^{U} {(\gamma_{F}^{u})}^2,
\end{aligned}
\end{equation}
where the penultimate inequality comes from Cauchy-Schwarz inequality: 
\begin{equation}
\Vert \sum_k a_k b_k\Vert^2 \leq \sum_{j} \Vert a_j\Vert^2 \sum_{k} \Vert b_k \Vert^2,
\end{equation}
with $a_j = \frac{1}{\sqrt{U}}$ and $b_k = \frac{1}{\sqrt{U}} (\nabla F_i(w_{k_1}(t-1)) - \frac{1}{W_k} \sum_{i =1}^{W_k}\nabla F_i(w_{k_1}(t-1)))$, and the final inequality comes from application of Lemma 4.4 from~\cite{fallah2020personalized}.

Returning to the original inequality and applying $(*)$ and Cauchy-Schwarz, we then get:
\begin{equation}
\begin{aligned}
& 4 \mathbb{E}\bigg[\Vert \eta_i(t-1) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \eta_i(t-1) \Vert^2 \bigg] + 4 \mathbb{E}\bigg[\Vert \nabla F_i(\mathbf{w}_{k_1}(t-1)) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \nabla F_i(\mathbf{w}_{k_1}(t-1)) \Vert^2\bigg] \\
& \leq 4 \mathbb{E}\bigg[\Vert \eta_i(t-1) - \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \eta_i(t-1) \Vert^2 \bigg] + 4 \frac{1}{U} \sum_{u=1}^{U} {(\gamma_{F}^{u})}^2 \\
& \leq 8 \mathbb{E}\bigg[\Vert \eta_i(t-1) \Vert^2 \bigg] + 8\frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \mathbb{E} \bigg[\Vert \eta_i(t-1) \Vert^2\bigg] + 4\frac{1}{U} \sum_{u=1}^{U} {(\gamma_{F}^{u})}^2.
\end{aligned}
\end{equation}

Now using Lemma 4.2 from~\cite{fallah2020personalized} and noting that average of average preservers Lipschitz gradient:
\begin{equation} \label{eq:l2_proof_trick_summations}
\begin{aligned}
& 8 \mathbb{E}\bigg[\Vert \eta_i(t-1) \Vert^2 \bigg] + 8\frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \mathbb{E} \bigg[\Vert \eta_i(t-1) \Vert^2\bigg] + 4\frac{1}{U} \sum_{u=1}^{U} {(\gamma_{F}^{u})}^2 \\
& \leq 8 L_{F}^2 \mathbb{E}\bigg[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert^2 \bigg] + 8 L_F^2 \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \mathbb{E} \bigg[\Vert \mathbf{w}_{k_1}^{i}(t-1) - \mathbf{w}_{k_1}(t-1) \Vert^2\bigg] + 4\frac{1}{U} \sum_{u=1}^{U} {(\gamma_{F}^{u})}^2 \\
& = 8 L_{F}^2 \Upsilon_i(t-1) + 8 L_F^2 \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \Upsilon_i(t-1) + 4\frac{1}{U} \sum_{u=1}^{U} {(\gamma_{F}^{u})}^2 
\end{aligned}
\end{equation}

Recall the sequence of summations in~\eqref{eq:l2_p1}, since the summations over $U$ and $W_u$ happen twice, the arguments of the inner summations become constants independent of $U$ and $W_u$ allowing us to express~\eqref{eq:l2_proof_trick_summations} as:
\begin{equation}
\begin{aligned}
&\frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \frac{1}{\tau_2} \sum_{k_1 = \tau_2(k_2 - 1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t = \tau_1 (k_1 -1)+1}^{\tau_1 k_1} \bigg[ 8 L_F^2 \Upsilon_i(t-1) + 8 L_F^2 \frac{1}{U} \sum_{\hat{u}=1}^{U} \frac{1}{W_{\hat{u}}} \sum_{i = 1}^{W_{\hat{u}}} \Upsilon_i(t-1) + 4\frac{1}{U} \sum_{\hat{u} \in \mathcal{U}} {(\gamma_{F}^{\hat{u}})}^2 \bigg] \\
&= \frac{1}{\tau_2} \sum_{k_1 = \tau_2(k_2 - 1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t = \tau_1 (k_1 -1)+1}^{\tau_1 k_1} \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \bigg[ 8 L_F^2 \Upsilon_i(t-1) + 8 L_F^2 \frac{1}{U} \sum_{\hat{u}=1}^{U} \frac{1}{W_{\hat{u}}} \sum_{i = 1}^{W_{\hat{u}}} \Upsilon_i(t-1) + 4\frac{1}{U} \sum_{\hat{u} \in \mathcal{U}} {(\gamma_{F}^{\hat{u}})}^2 \bigg] \\
&= \frac{1}{\tau_2} \sum_{k_1 = \tau_2(k_2 - 1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t = \tau_1 (k_1 -1)+1}^{\tau_1 k_1} \bigg[ \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} 16 L_{F}^2 \Upsilon_i(t-1) +4 \frac{1}{U} \sum_{u=1}^{U} {(\gamma_F^u)}^2\bigg].
\end{aligned}
\end{equation}

Using the above insight for $\Upsilon_i(t-1)$, combining~\eqref{eq:l2_proof_eqn_a} and~\eqref{eq:l2_proof_eqn_b}, and returning to~\eqref{eq:l2_proof_split} we obtain:
\begin{equation}
\begin{aligned}
&\frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \frac{1}{\tau_2} \sum_{k_1 = \tau_2(k_2 - 1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t = \tau_1 (k_1 -1)+1}^{\tau_1 k_1} \Upsilon_i(t)
= \frac{1}{\tau_2} \sum_{k_1 = \tau_2(k_2 - 1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t = \tau_1 (k_1 -1)+1}^{\tau_1 k_1} \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \Upsilon_i(t) \\
&\leq \frac{1}{\tau_2} \sum_{k_1 = \tau_2(k_2 - 1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t = \tau_1 (k_1 -1)+1}^{\tau_1 k_1} \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} (1+\phi)\Upsilon_i(t-1) \\
&+ \frac{1}{\tau_2} \sum_{k_1 = \tau_2(k_2 - 1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t = \tau_1 (k_1 -1)+1}^{\tau_1 k_1} \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} (1+\frac{1}{\phi}) \beta^2 \bigg[ 4 (\sigma_{F}^{u})^2 + 4 \frac{1}{U} \sum_{\hat{u}\in \mathcal{U}} \bigg((\sigma_{F}^{\hat{u}})^2 + (\gamma_{F}^{\hat{u}})^2 \bigg) + 16 L_{F}^2 \Upsilon_i(t-1)\bigg].
\end{aligned}
\end{equation}

Rearranging the above and excluding the summations for clarity gives:
\begin{equation}
\begin{aligned}
\Upsilon_i(t) \leq (1+\phi + 16(1+\frac{1}{\phi})\beta^2 L_F^2)\Upsilon_i(t-1) + 4(1+\frac{1}{\phi}) \beta^2 \bigg[ (\sigma_{F}^{u})^2 + \frac{1}{U} \sum_{\hat{u} \in \mathcal{U}} (\sigma_{F}^{\hat{u}})^2 + (\gamma_{F}^{\hat{u}})^2 \bigg],
\end{aligned}
\end{equation}

and, since the summation over time restricts $t$ such that $t\in \{\tau_1 (k_1-1)+1,\cdots,\tau_1 k_1 \}$ and at $t=k_1 \tau_1$ swarm aggregations occur, we have $\Upsilon_i(t)$:
\begin{equation}
\begin{aligned}
&\Upsilon_i(t) \leq (1+\phi + 16(1+\frac{1}{\phi})\beta^2 L_F^2)^{t - \tau_1 k_1} + 4(1+\frac{1}{\phi}) \beta^2 \bigg[ (\sigma_{F}^{u})^2 + \frac{1}{U} \sum_{\hat{u} \in \mathcal{U}} (\sigma_{F}^{\hat{u}})^2 + (\gamma_{F}^{\hat{u}})^2 \bigg] \sum_{y=0}^{t-(\tau_1 k_1)}(1+\phi + 16(1+\frac{1}{\phi})\beta^2 L_F^2)^y \\
&= (1+\phi + 16(1+\frac{1}{\phi})\beta^2 L_F^2)^{t - \tau_1 k_1} + 4(1+\frac{1}{\phi}) \beta^2 \bigg[ (\sigma_{F}^{u})^2 + \frac{1}{U} \sum_{\hat{u} \in \mathcal{U}} (\sigma_{F}^{\hat{u}})^2 + (\gamma_{F}^{\hat{u}})^2 \bigg] \frac{1-(1+\phi + 16(1+\frac{1}{\phi})\beta^2 L_F^2)^{t-k_1 \tau_1}}{1-(1+\phi + 16(1+\frac{1}{\phi})\beta^2 L_F^2)}
\end{aligned}
\end{equation}

Finally, reverting the form of $\Upsilon_i(t)$ and choosing $\phi =1$ gives:
\begin{equation}
\begin{aligned}
& \frac{1}{\tau_2} \sum_{k_1 = \tau_2(k_2 - 1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t = \tau_1 (k_1 -1)+1}^{\tau_1 k_1} \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \Upsilon_i(t) \leq \frac{1}{\tau_2} \sum_{k_1 = \tau_2(k_2 - 1)+1}^{\tau_2 k_2} \frac{1}{\tau_1} \sum_{t = \tau_1 (k_1 -1)+1}^{\tau_1 k_1} \frac{1}{U} \sum_{u=1}^{U} \frac{1}{W_u} \sum_{i = 1}^{W_u} \\
&\bigg[ (2 + 32\beta^2 L_F^2)^{t - \tau_1 k_1} + 8 \beta^2 \bigg[ (\sigma_{F}^{u})^2 + \frac{1}{U} \sum_{\hat{u} \in \mathcal{U}} (\sigma_{F}^{\hat{u}})^2 + (\gamma_{F}^{\hat{u}})^2 \bigg] \frac{1-(2 + 32\beta^2 L_F^2)^{t-k_1 \tau_1}}{1-(2 + 32\beta^2 L_F^2)} \bigg]
% &\bigg[ (1+\phi + 16(1+\frac{1}{\phi})\beta^2 L_F^2)^{t - \tau_1 k_1} + 4(1+\frac{1}{\phi}) \beta^2 \bigg[ (\sigma_{F}^{u})^2 + \frac{1}{U} \sum_{\hat{u} \in \mathcal{U}} (\sigma_{F}^{\hat{u}})^2 + (\gamma_{F}^{\hat{u}})^2 \bigg] \frac{1-(1+\phi + 16(1+\frac{1}{\phi})\beta^2 L_F^2)^{t-k_1 \tau_1}}{1-(1+\phi + 16(1+\frac{1}{\phi})\beta^2 L_F^2)} \bigg]
\end{aligned} 
\end{equation}

\end{proof}

==> old files/p2_v2.tex <==

\begin{proof} \label{sec:app_prop2} For convenience, the initial expression of Proposition~\ref{theory:prop_l2} appears as follows:
\begin{equation} \label{eq:prop2_eq1}
\begin{aligned}
&\mathbb{E}\bigg[ 
\bigg\Vert 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\bigg(\mathbf{w}^{i}(\tau_1 \tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2)
\bigg) 
\bigg\Vert^2
\bigg].
\end{aligned}
\end{equation}
The hierarchical relationships between $\mathbf{w}^i$ and $\mathbf{w}$ are unclear in~\eqref{eq:prop1_eq1}.
Therefore, we (a) introduce $\mathbf{w}^{u}$ terms, and (b) apply Jensen's inequality and use $\Vert a+b \Vert^2 \leq 2(\Vert a \Vert^2 + \Vert b \Vert^2)$ to separate the expression into separate relationships, mimicking the two-layer aggregation system of our problem:
\begin{equation} \label{eq:prop2_eq2}
\begin{aligned}
&\mathbb{E}\bigg[ 
\bigg\Vert 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\bigg(\mathbf{w}^{i}(\tau_1 \tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2)
\bigg) 
\bigg\Vert^2
\bigg] \\
& \overset{(a)}{=}
\mathbb{E}\bigg[ \bigg\Vert 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\bigg(\mathbf{w}^{i}(\tau_1 \tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) + \mathbf{w}^{u}(\tau_1 \tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2)
\bigg) 
\bigg\Vert^2
\bigg] \\
& \overset{(b)}{\leq}
2 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) \mathbb{E}[ \Vert 
\mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1\tau_2 k_2) 
\Vert^2 ] 
+ 2 \frac{1}{U}\sum_{u = 1}^{U}
\mathbb{E}[ \Vert 
\mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1\tau_2 k_2)
\Vert^2 ].
\end{aligned}
\end{equation}
The analysis of the two terms in~\eqref{eq:prop2_eq2} requires different techniques and so we perform their analyses separately. First, we upper bound $\mathbf{w}^{i}(\tau_1 \tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2)$ by recalling the meta-gradient update procedure at worker UAV $i$ and the local aggregation expression for $\mathbf{w}^{u}$, i.e., $\mathbf{w}^{u} (\tau_1 \tau_2 k_2) = \frac{1}{\Delta_u(k_2)}\sum_{i=1}^{W_u} \Delta_i(k_2) \mathbf{w}^{i} (\tau_1 \tau_2 k_2)$. 
Thus, omitting the summations for simplicity:
\begin{equation} \label{eq:prop2_eq3}
\begin{aligned} 
& \mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) \Vert^2 ]
= \mathbb{E} \bigg[ \bigg\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \frac{1}{\Delta_u(k_2)}\sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2)\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2) \bigg\Vert^2 \bigg] \\
& = \mathbb{E} \bigg[ \bigg\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2-1) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1))
- \frac{1}{\Delta_u(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}} (k_2) 
\bigg(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1) -\widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg)
\bigg\Vert^2 \bigg].
\end{aligned}
\end{equation}

\noindent
Already, we can see there exists a recursive relationship between $\mathbf{w}^{i}(\tau_1 \tau_2 k_2)$ and $\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)$. The relationship between the mini-batch meta-gradients is less clear however. To progress, we then compare the mini-batch meta-gradients $\widetilde{\nabla F_i}$ and $\widetilde{\nabla F_u} =  \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}$ with respect to the true gradients $\nabla F_i$ and $\nabla F_u = \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \nabla F_i$. 
Thus, we (a) introduce true gradients $\nabla F_i$ and $\nabla F_u$, and (b) apply $(\sum_i^n a_i)^2 \leq n(\sum_i^n a_i^2) $:
\begin{equation} \label{eq:prop2_eq4}
\begin{aligned}
&\mathbb{E} \bigg[ \bigg\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2-1) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1))
- \frac{1}{\Delta_u(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) 
\bigg(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1) -\widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg) 
\bigg\Vert^2 \bigg] \\
& \overset{(a)}{=} 
\mathbb{E} \bigg[ \bigg\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2-1) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1))
+ \nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1))
- \nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1))
\\
&
- \frac{1}{\Delta_u(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) 
\bigg(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1) 
- \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) 
+ \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) 
- \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) 
\bigg) 
\bigg\Vert^2 \bigg] 
\\
& \overset{(b)}{\leq}
4\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert^2 ]
+ 4\mathbb{E} [ \Vert 
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) 
\Vert^2 ] \\
& + 4\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{\Delta_u(k_2)} \sum_{\hat{i}=1}^{W_u} \Delta_{\hat{i}}(k_2) \bigg( \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) - \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg) 
\bigg\Vert^2 \bigg] \\
&+
4\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \frac{1}{\Delta_{u}(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert^2 \bigg].
\end{aligned}
\end{equation}

\noindent 
The $\mathbb{E}[\Vert \nabla F_i - \widetilde{\nabla F_i} \Vert^2]$ terms are easy to upper bound via Lemma~\ref{theory:lemma_sigma}. However, the final term in~\eqref{eq:prop2_eq4} poses two challenges: (i) the loss function gradients $\nabla F_i$ are on different datasets - hence entirely different loss functions, and (ii) the parameters $\mathbf{w}^{i}$ are unique for each worker UAV $i \in \mathcal{W}_u$. We address these two challenges in tandem by introducing $\nabla F_i(\mathbf{w}^u)$ and $\nabla F_{\hat{i}}(\mathbf{w}^u)$, which allows us to take advantage of the $\mu_F$-Lipschitz smooth property determined earlier in the main text.
For simplicity, we will first analyze the last term in~\eqref{eq:prop2_eq4} in isolation and then recombine its result with that of~\eqref{eq:prop2_eq4}. Hence:
\begin{equation} \label{eq:prop2_eq5}
\begin{aligned}
& 4\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \frac{1}{\Delta_{u}(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert^2 \bigg] \\
& = 
4\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
+ \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
\\
& 
- \frac{1}{\Delta_{u}(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) 
\bigg( 
\nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1)) 
+ \nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
- \nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg)
\bigg\Vert^2 \bigg].
\end{aligned}
\end{equation}
We now need to bring back the previously omitted summations from~\eqref{eq:prop2_eq3}. Then, starting from~\eqref{eq:prop2_eq5} with the summations, we (a) apply $(\sum_i^n a_i)^2 \leq n(\sum_i^n a_i^2) $, 
(b) both recall the form of $\nabla F_u$ and apply Jensen's inequality, 
(c) use $\mu_F$-Lipschitz smoothness (i.e., $\Vert \nabla F_i(\mathbf{w}) - \nabla F_i (\mathbf{w}') \Vert \leq \mu_F \Vert \mathbf{w} - \mathbf{w}' \Vert$ $\forall i \in \cup_{u \in \mathcal{U}} \mathcal{W}_u$), 
and (d) leverage Lemma~\ref{theory:lemma_gamma}, and thus obtain:
\begin{equation} \label{eq:prop2_eq6}
\begin{aligned}
%%%     (a)
& \overset{(a)}{\leq} 
12\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} [ \Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
\Vert^2 ]
\\
& + 12\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} \bigg[ \bigg\Vert  \frac{1}{\Delta_{u}(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) 
\bigg(
\nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
- \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1)) 
\bigg)
\bigg\Vert^2 \bigg] \\
& + 12\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} \bigg[ \bigg\Vert \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \frac{1}{\Delta_{u}(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) 
\nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg \Vert^2 \bigg] \\
%%%       (b)
& \overset{(b)}{\leq} 
12\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} [ \Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
\Vert^2 ]
\\
& + 12\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) \frac{1}{\Delta_{u}(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) 
\mathbb{E} \bigg[ \bigg\Vert  \nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) - \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}} (\tau_1\tau_2 k_2 -1))
\bigg\Vert^2 \bigg] \\
&
+ 12\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} \bigg[ \bigg\Vert \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_{u}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg \Vert^2 \bigg] \\
%%%       (c)
& \overset{(c)}{\leq} 
12 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) \mu_F^2
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 -1) \Vert^2 ]\\
& +
12 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) \frac{1}{\Delta_{u}(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) 
\mu_F^2 \mathbb{E} [ \Vert \mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1) - \mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2 -1) \Vert^2 ] \\
& + 
12 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} \bigg[ \bigg\Vert \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_{u}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg \Vert^2 \bigg] \\
%%%       (d)
& \overset{(d)}{\leq} 
24 \mu_F^2 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 -1) \Vert^2]
+
12\frac{1}{U} \sum_{u = 1}^{U} (\gamma_{F}^{u})^2.
\end{aligned}
\end{equation}

\noindent We return to~\eqref{eq:prop2_eq3} with the new results from~\eqref{eq:prop2_eq4} and~\eqref{eq:prop2_eq6}. Now, we (a) combine the result of~\eqref{eq:prop2_eq4} into~\eqref{eq:prop2_eq3} with the summations returning, (b) apply Jensen's inequality and Lemma 1, and (c) use the result in~\eqref{eq:prop2_eq6}. Hence, we obtain:
\begingroup
\allowdisplaybreaks
%\begin{equation}
\begin{align}
& \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) \Vert^2 ] \label{eq:prop2_eq7} \\
%%%     (a)
& \overset{(a)}{\leq} 
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert^2 ] 
\nonumber\\
& + 4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} [ \Vert 
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) 
\Vert^2 ] 
\nonumber\\
& + 4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{\Delta_u(k_2)} \sum_{\hat{i}=1}^{W_u} \Delta_{\hat{i}}(k_2) \bigg( \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) - \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg) 
\bigg\Vert^2 \bigg] \nonumber\\
&+ 4 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \frac{1}{\Delta_{u}(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert^2 \bigg] \nonumber\\
%%%         (b)
& \overset{(b)}{\leq}
4 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert^2 ] 
+ 8\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
(\sigma_F^{i}(\tau_1\tau_2 k_2 -1))^2
\nonumber\\
& + 
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \frac{1}{\Delta_{u}(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert^2 \bigg] \nonumber \\
%%%         (c)
& \overset{(c)}{\leq}
(4+ 24\mu_F^2)
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert^2 ] 
\nonumber\\
& + 8\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
(\sigma_F^{i}(\tau_1 \tau_2 k_2 -1))^2
+
12\frac{1}{U} \sum_{u = 1}^{U} (\gamma_{F}^{u})^2.
\nonumber
\end{align}
%\end{equation}
\endgroup

\noindent Comparing left and right hand sides of~\eqref{eq:prop2_eq7}, we see the recursive relationship between $\mathbb{E}[\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1\tau_2 k_2) \Vert^2]$ 
and 
$\mathbb{E}[\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2-1) - \mathbf{w}^{u}(\tau_1\tau_2 k_2-1) \Vert^2]$ emerge. 
In our problem formulation, swarm aggregations at some swarm $u$ occur among the swarm leader $z_u$ and its worker UAVs $i \in \mathcal{W}_u$ with period $\tau_1$. Therefore, $\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -\tau_1) = \mathbf{w}^{u}(\tau_1 \tau_2 k_2 - \tau_1)$. Performing the recursion on~\eqref{eq:prop2_eq7} for $\tau_1$ instances starting from $\tau_1 \tau_2 k_2$ thus yields:
\begin{equation}
\label{eq:prop2_eq8}
\begin{aligned}
& \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) \mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) \Vert^2 ] \\
& 
\leq 
8\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\bigg(
\sum_{y=0}^{\tau_1 -1}
(\sigma_F^{i}(\tau_1 \tau_2 k_2 - 1 -y))^2 (4+24\mu_F^2)^{y}
\bigg)
+
12 \frac{1}{U} \sum_{u = 1}^{U}(\gamma_{F}^{u})^2
\frac{1 - (4+24 \mu_F^2)^{\tau_1}}{1- (4+24\mu_F^2)}\\
&
\leq
\bigg(
8\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\sum_{y=0}^{\tau_1 -1}
(\sigma_F^{i}(\tau_1 \tau_2 k_2 - 1 -y))^2
+
12 \frac{1}{U} \sum_{u = 1}^{U}(\gamma_{F}^{u})^2
\bigg)
\frac{1 - (4+24 \mu_F^2)^{\tau_1}}{1- (4+24\mu_F^2)},
\end{aligned}
\end{equation}
where the last inequality comes from $\sum_i a_i b_i \leq \sum_i a_i \sum_i b_i$ $\forall a_i, b_i \geq 0$, and the finite sum of geometric series.
\noindent
We now proceed to analyze the second term in~\eqref{eq:prop2_eq2}, i.e., $\mathbb{E} [\Vert \mathbf{w}^{u}(\tau_1 \tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert^2]$. We begin by omitting the outer summations for clarity and expand the form of $\mathbf{w}$, which produces:
\begin{equation} \label{eq:prop2_eq9}
\begin{aligned}
& \mathbb{E} [ \Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert^2 ] 
= \mathbb{E} \bigg[ \bigg\Vert  \mathbf{w}^{u}(\tau_1\tau_2 k_2)
- \frac{1}{U} \sum_{\hat{u}=1}^{U} 
\mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2) \bigg\Vert^2 \bigg] \\
& =
\mathbb{E} \bigg[ \bigg\Vert  \mathbf{w}^{u}(\tau_1\tau_2 k_2-1)
- \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1))
- \frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2-1) 
- \widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
\bigg)
\bigg\Vert^2 \bigg].
\end{aligned}
\end{equation}

\noindent 
Similarly to the analysis of $\mathbb{E}[\Vert \mathbf{w}^{i} - \mathbf{w}^{u} \Vert^2 ]$ in~\eqref{eq:prop2_eq4}, we first compare the meta-gradients $\widetilde{\nabla F_u}$ against the true gradient $\nabla F_u$. Thus, starting from~\eqref{eq:prop2_eq9}, we (a) show an equivalent form and then (b) apply $(\sum_i^n a_i)^2 \leq n(\sum_i^n a_i^2) $:
\begin{equation} \label{eq:prop2_eq10}
\begin{aligned}
%%%         (a)
& \overset{(a)}{=}
\mathbb{E} \bigg[ \bigg\Vert  \mathbf{w}^{u}(\tau_1\tau_2 k_2-1)
- \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) 
+ \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
\\
&
- \frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2-1) 
- \widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
+ \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
\bigg)
\bigg\Vert^2 \bigg] \\
%%%         (b)
& \overset{(b)}{\leq} 
4\mathbb{E} \bigg[ \bigg\Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \frac{1}{U} \sum_{\hat{u} =1}^{U} \mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2 -1)
\bigg\Vert^2 \bigg]
+
4\mathbb{E} [ \Vert \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) \Vert^2 ]\\
& + 4\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)) 
\bigg)
\bigg\Vert^2 \bigg] \\
& + 4\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) \bigg\Vert^2 \bigg].
\end{aligned}
\end{equation}

\noindent
The middle two terms on the right hand side of~\eqref{eq:prop2_eq10} are easily bounded once we expand the hierarchy, use Jensen's inequality, and apply Lemma~\ref{theory:lemma_sigma}. As in~\eqref{eq:prop2_eq4}, the main challenge in~\eqref{eq:prop2_eq10} is the last term due to (i) the loss function gradients $\nabla F_u$ are on different datasets - hence entirely different loss functions, and (ii) the parameters $\mathbf{w}^{u}$ are unique for each swarm $u \in \mathcal{U}$. We address these two challenges in tandem by introducing $\nabla F_u(\mathbf{w})$ and $\nabla F_{\hat{u}}(\mathbf{w})$, which allows us to take advantage of both $\mu_F$-Lipschitz smooth property and Lemma~\ref{theory:lemma_gamma}. Hence:
\begin{align} \label{eq:prop2_eq11}
& 4\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
\bigg\Vert^2 \bigg] \nonumber \\
& = 
4\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}(\tau_1\tau_2 k_2-1))
+ \nabla F_{\hat{u}} (\mathbf{w}(\tau_1\tau_2 k_2-1))
\bigg)
\nonumber \\
& 
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
+ \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\bigg\Vert^2 \bigg].
\end{align}

\noindent
We now bound~\eqref{eq:prop2_eq10} which requires bringing back the previously omitted summations. Then, we 
(a) combine~\eqref{eq:prop2_eq10} and~\eqref{eq:prop2_eq11}, 
(b) expand the form of $\nabla F_{\hat{u}}$ into its constituent $\nabla F_{i}$, apply Jensen's inequality, and $(\sum_i^n a_i)^2 \leq n(\sum_i^n a_i^2) $,
(c) use Lemma~\ref{theory:lemma_sigma} and $\mu_F$-Lipschitz smooth,
and (d) expand the summations and use Lemma~\ref{theory:lemma_gamma}. For clarity, we explain from $\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert]$ as follows:
\begin{align} \label{eq:prop2_eq12}
& \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert^2] \nonumber\\
%%%     (a)
& \overset{(a)}{\leq}
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} \bigg[ \bigg\Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \frac{1}{U} \sum_{\hat{u} =1}^{U} \mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2 -1)
\bigg\Vert^2 \bigg] 
\nonumber \\
& +
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [ \Vert \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) \Vert^2 ] 
\nonumber \\
& + 
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)) 
\bigg)
\bigg\Vert^2 \bigg] 
\nonumber \\
& + 
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}(\tau_1\tau_2 k_2-1))
+ \nabla F_{\hat{u}} (\mathbf{w}(\tau_1\tau_2 k_2-1))
\nonumber \\
& 
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
+ \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\bigg\Vert^2 \bigg]
\bigg) 
\nonumber \\
%%%         (b)
& \overset{(b)}{\leq} 
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} \bigg[ \bigg\Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \frac{1}{U} \sum_{\hat{u} =1}^{U} \mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2 -1)
\bigg\Vert^2 \bigg] 
\nonumber \\
& + 
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{\Delta_u(k_2)} \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [ \Vert \nabla F_i (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \widetilde{\nabla F_i}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) \Vert^2 ] 
\nonumber \\
& + 
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \frac{1}{\Delta_{\hat{u}}(k_2)} \sum_{i = 1}^{W_{\hat{u}}} \Delta_i(k_2) 
\mathbb{E} [ \Vert
\widetilde{\nabla F_{i}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{i} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)) 
\Vert^2 ] 
\nonumber \\
& + 
12\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \frac{1}{\Delta_{\hat{u}}(k_2)} \sum_{i = 1}^{W_{\hat{u}}} \Delta_i(k_2) 
\mathbb{E} [ \Vert 
\nabla F_{i} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{i} (\mathbf{w}(\tau_1\tau_2 k_2-1))
\Vert^2 ]
\nonumber \\
& + 
12\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{\Delta_{u}(k_2)} \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [\Vert \nabla F_{i} (\mathbf{w}(\tau_1\tau_2 k_2-1))
- \nabla F_i (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
\Vert^2 ] 
\nonumber \\
& + 
12\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \nabla F_{\hat{u}} (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\bigg\Vert^2 \bigg]
\nonumber \\
%%%         (c)
& \overset{(c)}{\leq} 
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [ \Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}(\tau_1 \tau_2 k_2 -1)
\Vert^2 ] 
\nonumber \\
& + 
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{\Delta_u(k_2)} \sum_{i = 1}^{W_u} \Delta_i(k_2) 
(\sigma_F^i(\tau_1\tau_2 k_2 -1))^2 \nonumber \\
&
+
4\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \frac{1}{\Delta_{\hat{u}}(k_2)} \sum_{i = 1}^{W_{\hat{u}}} \Delta_i(k_2) 
(\sigma_F^i(\tau_1 \tau_2 k_2 -1))^2
\nonumber \\
& + 
12 \mu_F^2 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \frac{1}{\Delta_{\hat{u}}(k_2)} \sum_{i = 1}^{W_{\hat{u}}} \Delta_i(k_2) 
\mathbb{E} [ \Vert 
\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)
- \mathbf{w}(\tau_1\tau_2 k_2-1)
\Vert^2 ]
\nonumber \\
& + 
12 \mu_F^2 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\frac{1}{\Delta_{u}(k_2)} \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [\Vert \mathbf{w}(\tau_1\tau_2 k_2-1)
- \mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)
\Vert^2 ] 
\nonumber \\
& + 
12 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\mathbb{E} [\Vert 
\nabla F (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\Vert^2]
\nonumber \\
%%%         (d)
& \overset{(d)}{\leq} 
(4+ 24\mu_F^2) \frac{1}{U}\sum_{u = 1}^{U} \mathbb{E} [ \Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}(\tau_1 \tau_2 k_2 -1)
\Vert^2 ] \nonumber \\
&
+ 
8 \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
(\sigma_F^i(\tau_1 \tau_2 k_2 -1))^2
+ 12 \gamma_F^2.
\end{align}

\noindent 
Comparing left and right hand sides of~\eqref{eq:prop2_eq12}, we see the recursive relationship between $\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1\tau_2 k_2) \Vert]$ 
and 
$\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2-1) - \mathbf{w}(\tau_1\tau_2 k_2-1) \Vert^2]$ emerge. 
Differently from swarm aggregations, global aggregations among all swarm leaders $\{z_u\}$, $\forall u \in \mathcal{U}$ only occurs every $\tau_2$ swarm aggregations, i.e., every $\tau_1 \tau_2$ time instances. Therefore, $\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -\tau_1\tau_2) = \mathbf{w}(\tau_1 \tau_2 k_2 - \tau_1\tau_2)$. Performing the recursion on~\eqref{eq:prop2_eq12} for $\tau_1\tau_2$ instances starting from $\tau_1 \tau_2 k_2$ thus yields:
\begin{equation}
\label{eq:prop2_eq13}
\begin{aligned}
& 
\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)\mathbb{E} [ \Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert^2 ] 
=
\frac{1}{U}\sum_{u = 1}^{U} \mathbb{E} [ \Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert^2 ] 
\\
& \leq 
8\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\bigg(
\sum_{y=0}^{\tau_1\tau_2-1}(\sigma_F^{i}(\tau_1\tau_2 k_2-1-y))^2 (4+24\mu_F^2)^{y}
\bigg)
+
12 \gamma_{F}^2
\frac{1 - (4+24 \mu_F^2)^{\tau_1 \tau_2}}{1- (4+24\mu_F^2)} \\
& \leq
\bigg(
8\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\sum_{y=0}^{\tau_1\tau_2-1} (\sigma_F^{i}(\tau_1\tau_2 k_2-1-y))^2
+
12\gamma_{F}^2
\bigg)
\frac{1 - (4+24 \mu_F^2)^{\tau_1 \tau_2}}{1- (4+24\mu_F^2)},
\end{aligned}
\end{equation}
where the last inequality comes from $\sum_{i} a_i b_i \leq \sum_{i} a_i \sum_{i} b_i$ $\forall a_i, b_i \geq 0$ followed by the sum of finite geometric series.
Finally, combining the results of~\eqref{eq:prop2_eq8} and~\eqref{eq:prop2_eq13} back into~\eqref{eq:prop2_eq2} and shifting the summation from $y=0$ to $y=1$ yields the result:
\begin{equation}
\label{eq:prop2_eq14}
\begin{aligned}
& \frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\bigg( \mathbb{E}[\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1\tau_2 k_2) \Vert^2 ] + \mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1\tau_2 k_2)
\Vert^2] \bigg) \\
& \leq 
\bigg(
8\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2)
\sum_{y=1}^{\tau_1}
(\sigma_F^{i}(\tau_1 \tau_2 k_2 - y))^2
+
12 \frac{1}{U} \sum_{u = 1}^{U}(\gamma_{F}^{u})^2
\bigg)
\frac{1 - (4+24 \mu_F^2)^{\tau_1}}{1- (4+24\mu_F^2)}\\
& +
\bigg(
8\frac{1}{U}\sum_{u = 1}^{U} \frac{1}{\Delta_u(k_2)}  \sum_{i = 1}^{W_u} \Delta_i(k_2) 
\sum_{y=1}^{\tau_1\tau_2}(\sigma_F^{i}(\tau_1\tau_2 k_2-y))^2
+
12 \gamma_{F}^2
\bigg)
\frac{1 - (4+24 \mu_F^2)^{\tau_1 \tau_2}}{1- (4+24\mu_F^2)}.
\end{aligned}
\end{equation}

\end{proof}

==> old files/t1_proof_v1.tex <==
\begin{proof}
% \ali{to find a bound for the ..., we use .... obtain from prop ..., to this end, we first try to ...}
In order to find a bound for the first-order stationary point, $\mathbb{E}[ \Vert \nabla F(\mathbf{w}) \Vert^2]$, we want to use the known recursive relationship between $\mathbf{E}[ \Vert \mathbf{w}^i(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert^2]$, i.e., our proposition. How to apply proposition~\ref{theory:prop_l2} to isolate for $\mathbb{E}[\Vert \nabla F(\mathbf{w}) \Vert^2]$ is not clear however.
So, we recall that $F$, $F_u$, and $F_i$ are all $\mu_F$-Lipschitz smooth, and thus \ali{check how to call this}:
\begin{equation} \label{eq:theorem1_eq1}
\begin{aligned}
&F(\mathbf{w}(\tau_1\tau_2 k_2)) \leq F(\mathbf{w}(\tau_1\tau_2 k_2-1)) + \nabla F(\mathbf{w}(\tau_1\tau_2 k_2-1))^{T}(\mathbf{w}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1\tau_2 k_2-1)) + \frac{\mu_F}{2} \Vert \mathbf{w}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1\tau_2 k_2-1)\Vert^2 \\
& = 
F(\mathbf{w}(\tau_1\tau_2 k_2-1)) -\eta_2 \nabla F(\mathbf{w}(\tau_1\tau_2 k_2-1))^{T}
\bigg( \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1))\bigg) 
\\
& + \frac{\mu_F}{2} \bigg\Vert 
- \eta_2 \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1)) \bigg\Vert^2\\
& = 
F(\mathbf{w}(\tau_1\tau_2 k_2-1)) 
- \eta_2 \nabla F(\mathbf{w}(\tau_1\tau_2 k_2-1))^{T}
\bigg( \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}(\mathbf{w}^i(\tau_1\tau_2 k_2-1))\bigg) \\
&
+ \eta_2^2 \frac{\mu_F}{2} \bigg\Vert \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1)) \bigg\Vert^2.
\end{aligned}
\end{equation}

\noindent 
\ali{or, by taking ...} We take the expectation of both hand sides of~\eqref{eq:theorem1_eq1}, we can begin using Lemmas~\ref{theory:lemma_sigma} and~\ref{theory:lemma_gamma}, and Proposition~\ref{theory:prop_l2}. Later, we will extract the $\nabla F$ term from~\eqref{eq:theorem1_eq1} and leverage the recursive relationship between $F(\mathbf{w}(\tau_1 \tau_2 k_2))$ and $F(\mathbf{w}(\tau_1 \tau_2 k_2-1))$. 
Now, returning to~\eqref{eq:theorem1_eq1} and taking the expectation gives:
\begin{equation} \label{eq:theorem1_eq2}
\begin{aligned}
&\mathbb{E}[F(\mathbf{w}(\tau_1\tau_2 k_2))] 
\leq \mathbb{E}[F(\mathbf{w}(\tau_1\tau_2 k_2-1))] 
\\
& - \eta_2 \mathbb{E} \bigg[ 
\nabla F(\mathbf{w}(\tau_1\tau_2 k_2-1))^{T}
\bigg( \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}(\mathbf{w}^i(\tau_1\tau_2 k_2-1))\bigg) \bigg] \\
& + \eta_2^2 \frac{\mu_F}{2} \mathbb{E}\bigg[ \bigg\Vert 
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1))
\bigg\Vert^2 \bigg].
\end{aligned}
\end{equation}
% with
% \begin{equation}
% \begin{aligned}
% &(i) \triangleq \mathbb{E}\bigg[\nabla F(\mathbf{w}_{k_2}(t-1))^{T}\bigg( \frac{1}{U} \sum_{u \in \mathcal{U}} \frac{1}{W_{u}} \sum_{i \in \mathcal{W}_{u}} \widetilde{\nabla}F_i(\mathbf{w}_{k_2}^{i}(t-1))\bigg)\bigg]\\
% &(ii) \triangleq \mathbb{E}\bigg[\Vert \frac{1}{U} \sum_{u \in \mathcal{U}} \frac{1}{W_{u}} \sum_{i \in \mathcal{W}_{u}} \widetilde{\nabla}F_i(\mathbf{w}_{k_2}^{i}(t-1)) \Vert^2\bigg].
% \end{aligned}
% \end{equation}

\noindent
We begin by analyzing the second term on the right hand side (RHS) of~\eqref{eq:theorem1_eq2}. Analyzing $\widetilde{\nabla F_i}(\mathbf{w})$ directly is difficult, so we employ similar techniques as those of Proposition~\ref{theory:prop_l2} to obtain:
\begin{equation}\label{eq:theorem1_eq3}
\begin{aligned}
& \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}(\mathbf{w}^i(\tau_1\tau_2 k_2-1)) \\
& = 
X + Y + \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \nabla F_i(\mathbf{w}(\tau_1\tau_2 k_2-1)),
\end{aligned}
\end{equation}
where:
\begin{equation}
\begin{aligned}
& X \triangleq \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
\bigg[\widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1)) - \nabla F_i(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1)) \bigg]\\
& Y \triangleq \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2)
\bigg[\nabla F_i(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1)) - \nabla F_i(\mathbf{w}(\tau_1\tau_2 k_2-1)) \bigg].
\end{aligned}
\end{equation}

\noindent
Both $X$ and $Y$ are now in familiar formats as in the proof of Proposition~\ref{theory:prop_l2}. We first analyze $\Vert X \Vert^2$ using (a) Jensen's inequality, and (b) Lemma~\ref{theory:lemma_sigma} as follows:
\begin{equation} \label{eq:theorem1_eq4}
\begin{aligned}
&\mathbb{E}[\Vert X \Vert^2] = \mathbb{E}\bigg[ \bigg\Vert
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
\bigg( \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1)) - \nabla F_i(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1)) \bigg) \bigg\Vert^2 \bigg] \\
%%%%        (a)
&\overset{(a)}{\leq}
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
\mathbb{E}\bigg[ \Vert 
\widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1)) - \nabla F_i(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1))
\Vert^2 \bigg] \\
%%%%        (b)
&\overset{(b)}{\leq}
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(\tau_1\tau_2 k_2 -1))^2.
\end{aligned}
\end{equation}

\noindent
Next, we analyze $\Vert Y \Vert^2$  using (a) $\mu_{F}$-Lipschitz gradient property of $F_i$, and (b) Proposition~\ref{theory:prop_l2}. While Proposition~\ref{theory:prop_l2} may appear to bound $\Vert \mathbf{w}^i(\tau_1\tau_2k_2) - \mathbf{w}(\tau_1\tau_2k_2) \Vert^2$ only, the recursion in the bound is over an entire global interval $\tau_1\tau_2$, and hence Proposition~\ref{theory:prop_l2} also bounds $\Vert \mathbf{w}^i(\tau_1\tau_2k_2-c) - \mathbf{w}(\tau_1\tau_2k_2-c) \Vert^2$, $\forall c \in \{0,\cdots,\tau_1\tau_2\}$. Thus:
\begin{equation} \label{eq:theorem1_eq5}
\begin{aligned}
&\mathbb{E}[\Vert Y \Vert^2] = \mathbb{E}\bigg[ \bigg\Vert
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
\bigg( \nabla F_i(\mathbf{w}^{i}(\tau_1\tau_2k_2-1)) - \nabla F_i(\mathbf{w}(\tau_1\tau_2k_2-1)) \bigg) 
\bigg\Vert^2 \bigg] \\
& \overset{(a)}{\leq}
\mu_F^2 \mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
\bigg(
\mathbf{w}^{i}(\tau_1 \tau_2 k_2-1) - \mathbf{w}(\tau_1 \tau_2 k_2-1)
\bigg)
\bigg\Vert^2 \bigg] 
\\
& \overset{(b)}{\leq}
\mu_F^2 \Upsilon(k_2,\tau_1,\tau_2).
\end{aligned}
\end{equation}

\noindent
Returning to the original goal of bounding the second term on the RHS of~\eqref{eq:theorem1_eq2}, we upper bound it as follows:
\begin{equation}
\label{eq:theorem1_eq6}
\begin{aligned}
& - \eta_2 \mathbb{E} \bigg[
\nabla F(\mathbf{w}(\tau_1\tau_2k_2-1))^T 
\bigg(\frac{1}{U}\sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}(\mathbf{w}^i(\tau_1\tau_2k_2-1)) 
\bigg) \bigg] \\
%%%%            (a)
& \overset{(a)}{=}
- \eta_2 \mathbb{E} \bigg[\nabla F(\mathbf{w}(\tau_1\tau_2k_2-1))^T 
\bigg( X + Y + \frac{1}{U}\sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
\nabla F_i(\mathbf{w}(\tau_1\tau_2k_2 - 1))
\bigg) \bigg] \\
%%%%            (b)
& \overset{(b)}{=}
- \eta_2 \mathbb{E} \bigg[\nabla F(\mathbf{w}(\tau_1\tau_2k_2-1))^T 
\bigg( X + Y +
\nabla F(\mathbf{w}(\tau_1\tau_2k_2 - 1))
\bigg) \bigg] \\
%%%%            (c)
& \overset{(c)}{=}
- \eta_2 
\bigg(
\mathbb{E} [\nabla F(\mathbf{w}(\tau_1\tau_2k_2-1))^T 
(X + Y) ] + \mathbb{E} [\Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \Vert^2] 
\bigg)
\\
%%%%            (d)
& \overset{(d)}{\leq}
\frac{-\eta_2 }{2} \mathbb{E}[ \Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \Vert^2 ] 
+ \eta_2 \bigg( \mathbb{E} [\Vert X \Vert^2] + \mathbb{E}[\Vert Y \Vert^2]
\bigg)
\\
%%%%            (e)
& \overset{(e)}{\leq}
\frac{-\eta_2}{2} \mathbb{E}[ \Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \Vert^2 ] 
+ \eta_2
\bigg(
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(\tau_1\tau_2 k_2 -1))^2
+ \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2)
\bigg),
\end{aligned}
\end{equation}
where (a) comes from introducing $\nabla F_i(\mathbf{w}^i)$ and $\nabla F_i(\mathbf{w})$ terms, (b) is the definition of $\nabla F$, (c) follows from linearity of expectation, (d) is due to \ali{fix bug}
\begin{equation}
\label{eq:theorem1_eq7}
\begin{aligned}
& \mathbb{E}[ \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1))^T(X+Y) ] 
\leq \frac{1}{2} \mathbb{E}[ \Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \Vert^2 ] + \frac{1}{2} \mathbb{E}[\Vert X+Y\Vert^2] \\
& \leq
\frac{1}{2} \mathbb{E}[ \Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \Vert^2 ] + \mathbb{E}[\Vert X \Vert^2] + \mathbb{E}[\Vert Y\Vert^2],
\end{aligned}
\end{equation}
and therefore
\begin{equation}
\label{eq:theorem1_eq8}
\begin{aligned}
&\mathbb{E} [\nabla F(\mathbf{w}(\tau_1\tau_2k_2-1))^T 
(X + Y) ] + \mathbb{E} [\Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \Vert^2 ]
\\
&
\geq
\mathbb{E} [\Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \Vert^2 ] - 
\frac{1}{2} \mathbb{E}[ \Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \Vert^2 ] - \mathbb{E}[\Vert X \Vert^2] - \mathbb{E}[\Vert Y\Vert^2],
\end{aligned}
\end{equation}
and (e) applies the results of~\eqref{eq:theorem1_eq4} and~\eqref{eq:theorem1_eq5}.
Moving onto the last term on the RHS of~\eqref{eq:theorem1_eq2}, we (f) substitute the result from~\eqref{eq:theorem1_eq3}, (g) apply $(\sum_i^n a_i)^2 \leq n(\sum_i a_i^2)$, (h) combine the results of~\eqref{eq:theorem1_eq4} and~\eqref{eq:theorem1_eq5}, (i) introduce the global gradient $\nabla F$, (j) recall that $\nabla F = \frac{1}{U} \sum_{u=1}^{U} \nabla F_u$ and use $(\sum_i^n a_i)^2 \leq n(\sum_i a_i^2)$, and (k) apply Jensen's inequality and Lemma~\ref{theory:lemma_gamma} as follows:
\begin{align} \label{eq:theorem1_eq9}
& 
\mathbb{E}\bigg[ \bigg\Vert 
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}(\mathbf{w}^i(\tau_1\tau_2 k_2-1))
\bigg\Vert^2 \bigg] \\
%%%%        (f)
& \overset{(f)}{\leq}
\mathbb{E}\bigg[ \bigg\Vert 
X + Y + \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \nabla F_{i}(\mathbf{w}(\tau_1\tau_2 k_2-1))
\bigg\Vert^2 \bigg] \nonumber \\
%%%%        (g)
& \overset{(g)}{\leq}
3\mathbb{E}[ \Vert 
X \Vert^2]
+ 3\mathbb{E}[ \Vert
Y \Vert^2]
+ 3\mathbb{E} \bigg[ \bigg\Vert \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \nabla F_{i}(\mathbf{w}(\tau_1\tau_2 k_2-1))
\bigg\Vert^2 \bigg] \nonumber \\
%%%%        (h)
& \overset{(h)}{\leq}
3 \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(\tau_1\tau_2 k_2 -1))^2 
+ 3 \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2) \nonumber \\
&
+ 3\mathbb{E} \bigg[ \bigg\Vert \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \nabla F_{i}(\mathbf{w}(\tau_1\tau_2 k_2-1))
\bigg\Vert^2 \bigg] \nonumber \\
%%%%        (i)
& \overset{(i)}{\leq}
3 \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(\tau_1\tau_2 k_2 -1))^2 + 3 \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2) \nonumber \\
&
+ 3\mathbb{E} \bigg[ \bigg\Vert \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
\bigg(\nabla F_{i}(\mathbf{w}(\tau_1\tau_2 k_2-1)) - \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) +\nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \bigg)
\bigg\Vert^2 \bigg] \nonumber \\
%%%%        (j)
& \overset{(j)}{\leq}
3 \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(\tau_1\tau_2 k_2 -1))^2 + 3 \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2) \nonumber \\
&
+ 6\mathbb{E} \bigg[ \bigg\Vert \frac{1}{U} \sum_{u=1}^{U} \bigg( \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
\nabla F_{i}(\mathbf{w}(\tau_1\tau_2 k_2-1)) - \nabla F_u(\mathbf{w}(\tau_1\tau_2k_2-1)) \bigg) \bigg\Vert^2 \bigg]
+ 6 \mathbb{E} \bigg[ \bigg\Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1))
\bigg\Vert^2 \bigg] \nonumber \\
%%%%        (k)
& \overset{(k)}{\leq}
6\mathbb{E}[\Vert \nabla F(\mathbf{w}(\tau_1\tau_2 k_2-1)) \Vert^2 ] 
+ 3 \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(\tau_1\tau_2 k_2 -1))^2 + 3 \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2) 
+ 6 \frac{1}{U} \sum_{u=1}^{U} (\gamma_F^u)^2 \nonumber
\end{align}

% \noindent While the result in~\eqref{eq:theorem1_eq9} is directly applied to the second term on the RHS of~\eqref{eq:theorem1_eq2}, subtracting a single $\mathbb{E}[\Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1))\Vert^2]$ from~\eqref{eq:theorem1_eq6} also bounds the last term on the RHS of~\eqref{eq:theorem1_eq2}. Explicitly, and using the techniques from~\eqref{eq:theorem1_eq6}:
% \begin{align} \label{eq:theorem1_eq7}
% & \mathbb{E}\bigg[ \bigg\Vert 
% \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1\tau_2 k_2-1))
% \bigg\Vert^2 \bigg]  \\
% & \leq
% 6\mathbb{E}[\Vert \nabla F(\mathbf{w}(\tau_1\tau_2 k_2-1)) \Vert^2 ] 
% + 3 \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
% (\sigma_{F}^{i}(\tau_1\tau_2 k_2 -1))^2 + 3 \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2) 
% + 6 \frac{1}{U} \sum_{u=1}^{U} (\gamma_F^u)^2. \nonumber
% \end{align}
\noindent
Returning to~\eqref{eq:theorem1_eq2}, we combine the results of~\eqref{eq:theorem1_eq6} and~\eqref{eq:theorem1_eq9} to obtain:
\begin{equation} \label{eq:theorem1_eq10}
\begin{aligned}
&\mathbb{E}[F(\mathbf{w}(\tau_1\tau_2 k_2))] 
\leq \mathbb{E}[F(\mathbf{w}(\tau_1\tau_2 k_2-1))] \\
& -
\frac{\eta_2 }{2}
\mathbb{E}[ \Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \Vert^2 ] 
+ \eta_2
\bigg(
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(\tau_1\tau_2 k_2 -1))^2
+ \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2)
\bigg)
\\
& + \eta_2^2 \frac{\mu_F}{2} 
\bigg(6\mathbb{E}[\Vert \nabla F(\mathbf{w}(\tau_1\tau_2 k_2-1)) \Vert^2 ] 
+ 3 \frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(\tau_1\tau_2 k_2 -1))^2 + 3 \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2) 
+ 6 \frac{1}{U} \sum_{u=1}^{U} (\gamma_F^u)^2 \bigg)
\end{aligned}
\end{equation}

\noindent
\ali{with some algebraic steps, we get} the algebra in~\eqref{eq:theorem1_eq10} yields:
\begin{equation} \label{eq:theorem1_eq11}
\begin{aligned}
& \mathbb{E}[F(\mathbf{w}(\tau_1\tau_2 k_2))] 
- \mathbb{E}[F(\mathbf{w}(\tau_1\tau_2 k_2-1))] 
\leq 
(6\eta_2^2 \frac{\mu_F}{2} - \frac{\eta_2}{2})\mathbb{E}[\Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2-1)) \Vert^2] \\
&
+ (3\eta_2^2 \frac{\mu_F}{2} + \eta_2)
\bigg( 
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(\tau_1\tau_2 k_2 -1))^2 
+ \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2) 
\bigg)
+
3\eta_2^2 \mu_F \frac{1}{U} \sum_{u=1}^{U} (\gamma_F^u)^2 .
\end{aligned}
\end{equation}

\noindent
Since our goal from the beginning was to find an upper bound for the first-order stationary point, $\mathbb{E}[\Vert \nabla F(\mathbf{w}(t))\Vert^2]$, we now take the average of~\eqref{eq:theorem1_eq11} over all time $t$, which yields: \henry{add +1 to the intermediate summation and dont forget the fraction}
\begin{equation}
\label{eq:theorem1_eq12}
\begin{aligned}
& \frac{1}{\tau_1 \tau_2 K_2} \sum_{k_2=1}^{K_2} \sum_{k_1 = \tau_2 (k_2-1)+1}^{\tau_2 k_2} \sum_{t = \tau_1 (k_1-1)+1}^{\tau_1 k_1} 
\mathbb{E}[F(\mathbf{w}(t))] 
- \mathbb{E}[F(\mathbf{w}(t-1))] 
=
\frac{1}{\tau_1 \tau_2 K_2} (
\mathbb{E}[F(\mathbf{w}(\tau_1\tau_2 K_2))] 
- \mathbb{E}[F(\mathbf{w}(0))]
)
\\
& 
\leq 
\frac{1}{\tau_1 \tau_2 K_2} \sum_{k_2=1}^{K_2} \sum_{k_1 = \tau_2 (k_2-1)}^{\tau_2 k_2} \sum_{t = \tau_1 (k_1-1)+1}^{\tau_1 k_1} 
\bigg[(6\eta_2^2 \frac{\mu_F}{2} - \frac{\eta_2}{2})\mathbb{E}[\Vert \nabla F(\mathbf{w}(t-1)) \Vert^2] \\
&
+ (3\eta_2^2 \frac{\mu_F}{2} + \eta_2)
\bigg( 
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(t -1))^2 
+ \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2) 
\bigg)
+
3\eta_2^2 \mu_F \frac{1}{U} \sum_{u=1}^{U} (\gamma_F^u)^2 \bigg].
\end{aligned}
\end{equation}

\noindent 
We now rearrange~\eqref{eq:theorem1_eq12} using $\eta_2 < \frac{1}{6\mu_F}$ (i.e., to ensure that $(6\eta_2^2 \frac{\mu_F}{2} - \frac{\eta_2}{2}) < 0$)
to isolate for $\mathbb{E}[\Vert \nabla F(\mathbf{w}(\tau_1\tau_2k_2)-1) \Vert^2]$, and thus obtain:

% \henry{old stuff from here}
% Replacing all the above results in~\eqref{eq:t1_p2} yields:
% \begin{equation}
% \begin{aligned}
% &\mathbb{E}[F(\mathbf{w}_{k_2}(t))] \leq \mathbb{E}[F(\mathbf{w}_{k_2}(t-1))] -\beta \bigg[ \frac{5}{2} \mathbb{E}\bigg[\Vert \nabla F(\mathbf{w}_{k_2}(t-1)) \Vert^2 \bigg] + 2 \frac{1}{U} \sum_{u \in \mathcal{U}} \bigg( (\sigma_{F}^{u})^2 + (\gamma_{F}^{u})^2 \bigg) + 2 L_F^2 \hat{\Upsilon} \bigg] \\
% &+ \beta^2\frac{L_{F}}{2} \bigg[ 4\mathbb{E}\bigg[\Vert \nabla F(\mathbf{w}_{k_2}(t-1)) \Vert^2 \bigg] + 4\frac{1}{U} \sum_{u \in \mathcal{U}} \bigg( (\sigma_{F}^{u})^2 + (\gamma_{F}^{u})^2 \bigg) + 4 L_F^2 \hat{\Upsilon} \bigg],
% \end{aligned}
% \end{equation}
% with some algebraic manipulations, we get:
% \begin{equation}
% \begin{aligned}
% &\mathbb{E}[F(\mathbf{w}_{k_2}(t))] - \mathbb{E}[F(\mathbf{w}_{k_2}(t-1))] \leq (2\beta^2 L_{F} - \frac{5\beta}{2}) \mathbb{E}\bigg[\Vert \nabla F(\mathbf{w}_{k_2}(t-1)) \Vert^2 \bigg] \\
% &+ (2\beta^2 L_{F} - 2\beta) \bigg[\frac{1}{U} \sum_{u \in \mathcal{U}} \bigg( (\sigma_{F}^{u})^2 + (\gamma_{F}^{u})^2 \bigg) + L_F^2 \hat{\Upsilon} \bigg].
% \end{aligned}
% \end{equation}
% Taking the summation from both sides with respect to $k_2$, $k_1$, and $t$ gives:
% \begin{equation}
% \begin{aligned}
% &\sum_{k_2 = 1}^{K} \sum_{k_1 = \tau_2 (k_2-1)+1}^{\tau_2 k_2} \sum_{t = \tau_1 (k_1-1)+1}^{\tau_1 k_1} \bigg(\mathbb{E}[F(\mathbf{w}_{k_2}(t))] - \mathbb{E}[F(\mathbf{w}_{k_2}(t-1))] \bigg) = \mathbb{E}[F(\mathbf{w}_{k_2}(\tau_2 \tau_1 K))] - \mathbb{E}[F(\mathbf{w}_{k_2}(0))] \\
% &\leq \sum_{k_2 = 1}^{K} \sum_{k_1 = \tau_2 (k_2-1)+1}^{\tau_2 k_2} \sum_{t = \tau_1 (k_1-1)+1}^{\tau_1 k_1}
% \bigg( (2\beta^2 L_{F} - \frac{5\beta}{2}) \mathbb{E}\bigg[\Vert \nabla F(\mathbf{w}_{k_2}(t-1)) \Vert^2 \bigg] \\
% &+ (2\beta^2 L_{F} - 2\beta) \bigg[\frac{1}{U} \sum_{u \in \mathcal{U}} \bigg( (\sigma_{F}^{u})^2 + (\gamma_{F}^{u})^2 \bigg) + L_F^2 \hat{\Upsilon} \bigg] \bigg).
% \end{aligned}
% \end{equation}
\begin{align} \label{eq:theorem1_eq13}
&-\frac{6\eta_2^2 \frac{\mu_F}{2} - \frac{\eta_2}{2}}{\tau_1 \tau_2 K_2}
\sum_{k_2=1}^{K_2} \sum_{k_1 = \tau_2 (k_2-1)}^{\tau_2 k_2} \sum_{t = \tau_1 (k_1-1)+1}^{\tau_1 k_1} 
\mathbb{E}[\Vert \nabla F(\mathbf{w}(t-1)) \Vert^2] \\
& \leq
\mathbb{E}[F(\mathbf{w}(0))]  
-
\mathbb{E}[F(\mathbf{w}(\tau_1\tau_2 K_2))] 
+ 
\frac{1}{\tau_1 \tau_2 K_2}
\sum_{k_2=1}^{K_2} \sum_{k_1 = \tau_2 (k_2-1)}^{\tau_2 k_2} \sum_{t = \tau_1 (k_1-1)+1}^{\tau_1 k_1} \nonumber \\
&
\bigg[
(3\eta_2^2 \frac{\mu_F}{2} + \eta_2)
\bigg( 
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(t -1))^2 
+ \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2) 
\bigg)
+
3\eta_2^2 \mu_F \frac{1}{U} \sum_{u=1}^{U} (\gamma_F^u)^2
\bigg]. \nonumber
\end{align}

Finally, noting that $\mathbb{E}[F(\mathbf{w}(0))] = F(\mathbf{w}(0))$ and that $-\mathbb{E}[F(\mathbf{w}(\tau_1 \tau_2 K_2))] \leq -F^*$, we have the result:
\begin{equation} \label{eq:theorem1_eq14}
\begin{aligned}
&
\frac{1}{\tau_1 \tau_2 K_2}
\sum_{k_2=1}^{K_2} \sum_{k_1 = \tau_2 (k_2-1)}^{\tau_2 k_2} \sum_{t = \tau_1 (k_1-1)+1}^{\tau_1 k_1} 
\mathbb{E}[\Vert \nabla F(\mathbf{w}(t-1)) \Vert^2] 
\leq 
\frac{1}{\frac{\eta_2}{2} - 6\eta_2^2 \frac{\mu_F}{2}}
\bigg[
F(\mathbf{w}(0)) - F^*
+ 
\frac{1}{\tau_1 \tau_2 K_2}
\sum_{k_2=1}^{K_2} \sum_{k_1 = \tau_2 (k_2-1)}^{\tau_2 k_2} \\
&
\sum_{t = \tau_1 (k_1-1)+1}^{\tau_1 k_1} 
\bigg[
(3\eta_2^2 \frac{\mu_F}{2} + \eta_2)
\bigg( 
\frac{1}{U} \sum_{u=1}^{U} \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) 
(\sigma_{F}^{i}(t -1))^2 
+ \mu_F^2 \Upsilon(k_2,\tau_1,\tau_2) 
\bigg)
+
3\eta_2^2 \mu_F \frac{1}{U} \sum_{u=1}^{U} (\gamma_F^u)^2
\bigg]
\bigg]
\end{aligned}
\end{equation}
\end{proof}



==> p1_updated.tex <==
\begin{proposition}[Expected worker-global parameter divergence]\label{theory:prop_l1}%[Expected parameter divergence among worker UAVs $j \in \cup_{u \in \mathcal{U}} \mathcal{W}_u$ compared to global average at $\mathsf{AP}$, ($\mathbf{w}_j$ vs. $\mathbf{w}$)] 
For $t$ within some global aggregation period, i.e., $t \in \{\tau_{s,1}\tau_{s,2} (k_{s,2}-1)+1, \cdots, \tau_{s,1}\tau_{s,2} k_{s,2} \}$, the expected average divergence of worker parameters $\mathbf{w}_j$, where $j \in \mathcal{W}_u$ $\forall u \in \mathcal{U}(t_s)$, is bounded w.r.t. the global average $\mathbf{w}$ at the core network.
\begin{align}
&\mathbb{E} \bigg[\bigg\Vert \frac{1}{U} \sum_{u \in \mathcal{U}} \sum_{j\in \mathcal{W}_u} \frac{\Delta_j(k_{s,2}) }{\Delta_u(k_{s,2})} 
\bigg( \mathbf{w}_j(t) - \mathbf{w}(t))
\bigg) \bigg\Vert \bigg] \leq \\
&
\bigg(
2 \eta_2 \frac{1}{U}\sum_{u \in \mathcal{U}} \sum_{j \in \mathcal{W}_u} \frac{\Delta_j(k_{s,2}) }{\Delta_u(k_{s,2})}
\sum_{y=1}^{\tau_{s,1}}
\sqrt{\sigma_i^{\mathsf{F}}(\tau_{s,1} \tau_{s,2} k_{s,2} - y)}
+
\eta_2
\frac{1}{U} \sum_{u \in \mathcal{U}} \sqrt{\gamma_u^{\mathsf{F}}}
\bigg)
\frac{1 - (1+2 \eta_2 \mu_F)^{\tau_{s,1}}}{1- (1+2 \eta_2 \mu_F)}
\nonumber \\
&+
\bigg(
2 \eta_2 \frac{1}{U}\sum_{u \in \mathcal{U}} \sum_{j \in \mathcal{W}_u} \frac{\Delta_j(k_{s,2}) }{\Delta_u(k_{s,2})}
\sum_{y=1}^{\tau_{s,1}\tau_{s,2}} \sqrt{\sigma_i^{\mathsf{F}}(\tau_{s,1}\tau_{s,2} k_{s,2}-y)}
+
\eta_2 \sqrt{\gamma_{F}}
\bigg)
\frac{1 - (1+2 \eta_2 \mu_F)^{\tau_{s,1} \tau_{s,2}}}{1- (1+2\eta_2 \mu_F)}. \nonumber
\end{align}

\begin{proof}
The proof is in Appendix~\ref{sec:app_prop1}
\end{proof}

% \input{l1_proof.tex}
\end{proposition}
% \begin{remark} [Proposition 1 with $\tau_2=1$]
% When the global aggregation period is $\tau_2 = 1$, then effectively the system becomes a two-layer system. For such a case, Proposition 1 devolves back into the classic result in~\cite{fallah2020personalized}.
% \end{remark}


\begin{proof} \label{sec:app_prop1} 
To bound
\begin{equation} \label{eq:prop1_eq1}
\begin{aligned}
&\mathbb{E}\bigg[ \bigg\Vert \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u}  \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\bigg(\mathbf{w}^{i}(\tau_1 \tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2)
\bigg) \bigg\Vert \bigg],
\end{aligned}
\end{equation}
where $\Delta_i(k_2) = \sum_{t = \tau_1 \tau_2 k_2 - \tau_1}^{\tau_1 \tau_2 k_2} \Delta_i(t)$, 
and $\Delta_u(k_2) = \sum_{i=1}^{W_u} \Delta_i(k_2)$, we 
% The hierarchical relationships between $\mathbf{w}^i$ and $\mathbf{w}$ are unclear in~\eqref{eq:prop1_eq1}. 
introduce $\mathbf{w}^{u}(\tau_1\tau_2k_2)$, which yields:
% to separate the expression into two separate relationships, mimicking the two-layer aggregation system of our problem:
\begin{equation} \label{eq:prop1_eq2}
\begin{aligned}
&\mathbb{E}\bigg[ \bigg\Vert 
\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\bigg(\mathbf{w}^{i}(\tau_1 \tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) + \mathbf{w}^{u}(\tau_1 \tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2)
\bigg) 
\bigg\Vert \bigg] \\
&\leq 
\underbrace{\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E}[\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1\tau_2 k_2) \Vert ]  }_{(i)}
+ 
\underbrace{
\frac{1}{U}\sum_{u = 1}^{U}
\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1\tau_2 k_2)
\Vert]}_{(ii)}.
\end{aligned}
\end{equation} 

\noindent
% The analysis of the two terms in~\eqref{eq:prop1_eq2} requires different techniques and so we perform their analyses separately. 
% First, we upper bound $\mathbf{w}^{i}(\tau_1 \tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2)$ by recalling the meta-gradient update procedure at worker UAV $i$ and the local aggregation expression for $\mathbf{w}^{u}$, i.e., $\mathbf{w}^{u} (\tau_1 \tau_2 k_2) = \frac{1}{\Delta_u(k_2)}\sum_{i=1}^{W_u} \Delta_i(k_2) \mathbf{w}^{i} (\tau_1 \tau_2 k_2)$. 
% Thus, omitting the outer summations, we obtain:
We first upper bound~\eqref{eq:prop1_eq2}(i), omitting the summations for simplicity:
\begin{equation} \label{eq:prop1_eq3}
\begin{aligned} 
& \mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) \Vert ]
\overset{(a)}{=} \mathbb{E} \bigg[ \bigg\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_u(k_2)} \mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2) \bigg\Vert \bigg] \\
& \overset{(b)}{=} \mathbb{E} \bigg[ \bigg\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2-1) - \eta_2 \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1))
- \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}} (k_2) }{\Delta_u(k_2)} 
\bigg(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1) - \eta_2 \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg)
\bigg\Vert \bigg] \\
% \end{aligned}
% \end{equation}
% \noindent
% Already, we can see there exists a recursive relationship between $\mathbf{w}^{i}(\tau_1 \tau_2 k_2)$ and $\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)$. The relationship between the mini-batch meta-gradients is less clear however. To progress, we then compare the mini-batch meta-gradients $\widetilde{\nabla F_i}$ and $\widetilde{\nabla F_u} =  \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \widetilde{\nabla F_i}$ with respect to the true gradients $\nabla F_i$ and $\nabla F_u = \frac{1}{\Delta_u(k_2)} \sum_{i=1}^{W_u} \Delta_i(k_2) \nabla F_i$. Thus:
% \begin{equation} \label{eq:prop1_eq4}
% \begin{aligned}
% &\mathbb{E} \bigg[ \bigg\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2-1) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1))
% - \frac{1}{\Delta_u(k_2)} \sum_{\hat{i} = 1}^{W_u} \Delta_{\hat{i}}(k_2) 
% \bigg(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1) -\widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg) 
% \bigg\Vert \bigg] \\
& \overset{(c)}{\leq} 
\underbrace{\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert ]}_{(i)}
+ 
\underbrace{\eta_2 
\mathbb{E} [ \Vert 
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) 
\Vert ]}_{(ii)} \\
& + 
\underbrace{\eta_2 
\mathbb{E} \bigg[ \bigg\Vert 
\sum_{\hat{i}=1}^{W_u} \frac{\Delta_{\hat{i}}(k_2) }{\Delta_u(k_2)} \bigg( \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) - \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg) 
\bigg\Vert \bigg]}_{(iii)} \\
&+
\underbrace{\eta_2 
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2) }{\Delta_{u}(k_2)} \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert \bigg]}_{(iv)},
\end{aligned}
\end{equation}
where $(a)$ is the aggregation rule of $\mathbf{w}^u$, $(b)$ uses the gradient update from~\eqref{eq:meta_gradient_update}, and $(c)$ introduces $\eta_2 \nabla F_i$ and $\eta_2 \nabla F_u$ terms and then applies triangle inequality. 
The bounds for~\eqref{eq:prop1_eq3}(ii) and~\eqref{eq:prop1_eq3}(iii) follow immediately from Lemma~\ref{theory:lemma_sigma}, and we analyze~\eqref{eq:prop1_eq3}(iv), while recalling the summations from~\eqref{eq:prop1_eq2} as follows:
% We use Lemma~\ref{theory:lemma_sigma} to bound~\eqref{prop1_eq3}(ii) and~\eqref{prop1_eq3}(iii). 
% \noindent
% The $\mathbb{E}[\Vert \nabla F_i - \widetilde{\nabla F_i} \Vert]$ terms are easy to upper bound via Lemma~\ref{theory:lemma_sigma}. However, the final term in~\eqref{eq:prop1_eq4} poses two challenges: (i) the loss function gradients $\nabla F_i$ are on different datasets - hence entirely different loss functions, and (ii) the parameters $\mathbf{w}^{i}$ are unique for each worker UAV $i \in \mathcal{W}_u$. We address these two challenges in tandem by introducing $\nabla F_i(\mathbf{w}^u)$ and $\nabla F_{\hat{i}}(\mathbf{w}^u)$, which allows us to take advantage of the $\mu_F$-Lipschitz smooth property determined earlier in the main text.
% For simplicity, we will first analyze the last term in~\eqref{eq:prop1_eq4} in isolation and then recombine its result with that of~\eqref{eq:prop1_eq4}.
\begin{align} \label{eq:prop1_eq4}
% \begin{aligned}
& \eta_2 
\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)}  \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert \bigg] \\ \nonumber
%%%%        (a)
& \overset{(a)}{=}
\eta_2 
\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
+ \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
\\ \nonumber
& 
- \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)} 
\bigg( 
\nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1)) 
+ \nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
- \nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg)
\bigg\Vert \bigg] \\ \nonumber
% \end{aligned}
% \end{equation}
% \begin{equation} \label{eq:prop1_eq6}
% \begin{aligned}
%%%     (b)
& \overset{(b)}{\leq} 
\eta_2\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
\Vert ]
\\ \nonumber
& + \eta_2
\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} \bigg[ \bigg\Vert  \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)}
\bigg(
\nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
- \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1)) 
\bigg)
\bigg\Vert \bigg] \\ \nonumber
& + \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\mathbb{E} \bigg[ \bigg\Vert \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2) }{\Delta_{u}(k_2)} 
\nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg \Vert \bigg] \\ \nonumber
%%%       (c)
& \overset{(c)}{\leq} 
\eta_2\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
\Vert ]
\\ \nonumber
& + 
\eta_2
\frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)}
\mathbb{E} \bigg[ \bigg\Vert 
\nabla F_{\hat{i}}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
- \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1)) 
\bigg\Vert \bigg]
\\ \nonumber
& 
+ \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\mathbb{E} \bigg[ \bigg\Vert \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_{u}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg \Vert \bigg] \\ \nonumber
%%%       (d)
& \overset{(d)}{\leq} 
\eta_2 \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} \mu_F 
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 -1) \Vert]
\\ \nonumber
& +
\eta_2
\frac{1}{U}\sum_{u = 1}^{U} %\sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)}
\mu_F 
\mathbb{E} [ \Vert \mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1) - \mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2 -1) \Vert ] 
\\ \nonumber
& 
+ \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\mathbb{E} \bigg[ \bigg\Vert \nabla F_i(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \nabla F_{u}(\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1))
\bigg \Vert \bigg]  \\ \nonumber
%%%       (e)
& \overset{(e)}{\leq} 
2 \mu_F \eta_2 \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 -1) \Vert]
+
\eta_2 \frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u},
\end{align}
% \end{equation}
where (a) introduces $\nabla F_i(\mathbf{w}^u)$ and $\nabla F_{\hat{i}}(\mathbf{w}^u)$,
(b) applies triangle inequality, 
(c) recalls the aggregation rule of $\nabla F_u$ and applies triangle inequality, 
(d) uses $\mu_F$-smoothness (i.e., $\Vert \nabla F_i(\mathbf{w}) - \nabla F_i (\mathbf{w}') \Vert \leq \mu_F \Vert \mathbf{w} - \mathbf{w}' \Vert$ $\forall i \in \cup_{u \in \mathcal{U}} \mathcal{W}_u$), 
and (e) leverages Lemma~\ref{theory:lemma_gamma}.
Combining~\eqref{eq:prop1_eq3} and~\eqref{eq:prop1_eq4} yields: 
%Now, we (a) combine the result of~\eqref{eq:prop1_eq4} into~\eqref{eq:prop1_eq3} with the summations returning, (b) apply triangle inequality and Lemma 1, and (c) use the result in~\eqref{eq:prop1_eq6}. Hence, we obtain:
\begingroup
\allowdisplaybreaks
%\begin{equation} 
\begin{align}
& \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) \Vert ] \label{eq:prop1_eq5} \\
%%%     (a)
& \overset{(a)}{\leq} 
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert ] \nonumber\\
& + \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert 
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) - \widetilde{\nabla F_i}(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1)) 
\Vert ] \nonumber\\
& + \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} \bigg[ \bigg\Vert 
\sum_{\hat{i}=1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_u(k_2)} \bigg( \widetilde{\nabla F_{\hat{i}}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) - \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1 \tau_2 k_2-1)) \bigg) 
\bigg\Vert \bigg] \nonumber\\
&+ \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2)}{\Delta_{u}(k_2)} \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert \bigg] \nonumber\\
%%%         (b)
& \overset{(b)}{\leq}
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert ] 
+ 
2 \eta_2 \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\sigma_F^{i}(\tau_1\tau_2 k_2 -1)
\nonumber\\
& + \eta_2
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} \bigg[ \bigg\Vert  
\nabla F_i(\mathbf{w}^{i}(\tau_1 \tau_2 k_2 -1)) - \sum_{\hat{i} = 1}^{W_u} \frac{\Delta_{\hat{i}}(k_2) }{\Delta_{u}(k_2)} \nabla F_{\hat{i}}(\mathbf{w}^{\hat{i}}(\tau_1\tau_2 k_2 - 1))
\bigg\Vert \bigg] \nonumber \\
%%%         (c)
& \overset{(c)}{\leq}
(1+ 2 \eta_2 \mu_F)
\frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}^{u} (\tau_1 \tau_2 k_2 - 1) \Vert ] 
\nonumber\\
& + 2\eta_2  \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)}  
\sigma_F^{i}(\tau_1 \tau_2 k_2 -1)
+
\eta_2
\frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u},
\nonumber
\end{align}
%\end{equation}
\endgroup
where $(a)$ restates~\eqref{eq:prop1_eq3} with the previously omitted summations, $(b)$ applies triangle inequality and Lemma~\ref{theory:lemma_sigma}, and $(c)$ uses the result in~\eqref{eq:prop1_eq4}. Solving~\eqref{eq:prop1_eq5} recursively yields:
\begin{align} \label{eq:prop1_eq6}
& \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2) }{\Delta_u(k_2)}  \mathbb{E} [ \Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1 \tau_2 k_2) \Vert ] \\
& 
%%%%        (a)
\overset{(a)}{\leq }
2 \eta_2 \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u}  \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\bigg(
\sum_{y=0}^{\tau_1 -1}
\sigma_F^{i}(\tau_1 \tau_2 k_2 - 1 -y) (1+2\eta_2\mu_F)^{y}
\bigg)
+ \eta_2
\frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u}
\frac{1 - (1+2 \eta_2 \mu_F)^{\tau_1}}{1- (1+2\eta_2\mu_F)}\\
&
%%%%        (b)
\overset{(b)}{\leq}
\bigg(
2 \eta_2 \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u}  \frac{\Delta_i(k_2)}{\Delta_u(k_2)}
\sum_{y=0}^{\tau_1 -1}
\sigma_F^{i}(\tau_1 \tau_2 k_2 - 1 -y)
+
\eta_2 \frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u}
\bigg)
\frac{1 - (1+2 \eta_2 \mu_F)^{\tau_1}}{1- (1+2 \eta_2 \mu_F)},
\end{align}
where $(a)$ is the result of recursion and the finite sum of geometric series, and $(b)$ uses $\sum_i a_i b_i \leq \sum_i a_i \sum_i b_i$ $\forall a_i, b_i \geq 0$. 
%%%%            Part 2 - the second term
Next, we bound~\eqref{eq:prop1_eq2}(ii) as follows:
\begin{equation} \label{eq:prop1_eq7}
\begin{aligned}
& \frac{1}{U} \sum_{u=1}^{U} 
\mathbb{E} [ \Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert ] 
%%%%        (a)
\overset{(a)}{=} \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert  \mathbf{w}^{u}(\tau_1\tau_2 k_2)
- \frac{1}{U} \sum_{\hat{u}=1}^{U} 
\mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2) \bigg\Vert \bigg] \\
%%%%        (b)
& \overset{(b)}{=}
\frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert  \mathbf{w}^{u}(\tau_1\tau_2 k_2-1)
- \eta_2 \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1))
- \frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2-1) 
- \eta_2 \widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
\bigg)
\bigg\Vert \bigg] \\
% Similarly to the analysis of $\mathbb{E}[\Vert \mathbf{w}^{i} - \mathbf{w}^{u} \Vert ]$ in~\eqref{eq:prop1_eq4}, we first compare the meta-gradients $\widetilde{\nabla F_u}$ against the true gradient $\nabla F_u$. Thus, starting from~\eqref{eq:prop1_eq9}, we (a) show an equivalent form and then (b) apply triangle inequality to simplify analysis:
%%%         (c)
& \overset{(c)}{=}
\frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert  \mathbf{w}^{u}(\tau_1\tau_2 k_2-1)
- \eta_2 \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) 
+ \eta_2 \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
- \eta_2 \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
\\
&
- \frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2-1) 
- \eta_2 \widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
+ \eta_2 \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \eta_2 \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
\bigg)
\bigg\Vert \bigg] \\
%%%         (d)
& \overset{(d)}{\leq} 
\underbrace{
\frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \frac{1}{U} \sum_{\hat{u} =1}^{U} \mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2 -1)
\bigg\Vert \bigg]}_{(i)}
+
\underbrace{
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} [ \Vert \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) \Vert ]
}_{(ii)}
\\
& + 
\underbrace{
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)) 
\bigg)
\bigg\Vert \bigg]}_{(iii)} \\
& + 
\underbrace{
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) \bigg\Vert \bigg]}_{(iv)},
\end{aligned}
\end{equation}

\noindent
where $(a)$ uses the definition of $\mathbf{w}$ from~\eqref{eq:global_wide_aggregation}, $(b)$ is the global parameter update rule from~\eqref{eq:pfl_meta_function_global_avg}, $(c)$ introduces $\eta_2 \nabla F_u(\mathbf{w}^u)$ and $\eta_2 \nabla F_{\hat{u}}(\mathbf{w}^{\hat{u}})$, and $(d)$ follows from triangle inequality. Upper bounds for~\eqref{eq:prop1_eq7}(ii) and~\eqref{eq:prop1_eq7}(iii) follow immediately from~\eqref{eq:pfl_meta_function_swarm_avg} and Lemma~\ref{theory:lemma_sigma}, and we bound~\eqref{eq:prop1_eq7}(iv) as follows:
% The middle two terms on the right hand side of~\eqref{eq:prop1_eq10} are easily bounded once we expand the hierarchy and apply Lemma~\ref{theory:lemma_sigma}. As in~\eqref{eq:prop1_eq4}, the main challenge in~\eqref{eq:prop1_eq10} is the last term due to (i) the loss function gradients $\nabla F_u$ are on different datasets - hence entirely different loss functions, and (ii) the parameters $\mathbf{w}^{u}$ are unique for each swarm UAV $u \in \mathcal{U}$. We address these two challenges in tandem by introducing $\nabla F_u(\mathbf{w})$ and $\nabla F_{\hat{u}}(\mathbf{w})$, which allows us to take advantage of both $\mu_F$-Lipschitz smooth property and Lemma~\ref{theory:lemma_gamma}. Hence:
\begin{align} \label{eq:prop1_eq8}
& 
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
\bigg\Vert \bigg] \nonumber \\
%%%%        (a)
& \overset{(a)}{=} 
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}(\tau_1\tau_2 k_2-1))
+ \nabla F_{\hat{u}} (\mathbf{w}(\tau_1\tau_2 k_2-1))
\bigg)
\nonumber \\
& 
- \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1))
+ \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
- \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\bigg\Vert \bigg] \nonumber \\
%%%%        (b)
& \overset{(b)}{\leq}
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[\bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \sum_{i=1}^{W_{\hat{u}}} \frac{\Delta_i(k_2)}{\Delta_{\hat{u}}(k_2)}
\bigg( \nabla F_i(\mathbf{w}^{\hat{u}}(\tau_1\tau_2k_2-1)) - \nabla F_i(\mathbf{w}(\tau_1\tau_2k_2-1)) \bigg)
\bigg\Vert \bigg]
\nonumber \\
& +
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[\bigg\Vert 
\sum_{i=1}^{W_{\hat{u}}} \frac{\Delta_i(k_2)}{\Delta_{\hat{u}}(k_2)} 
\bigg( \nabla F_i(\mathbf{w}(\tau_1\tau_2k_2-1)) - \nabla F_i(\mathbf{w}^{u}(\tau_1\tau_2k_2-1)) \bigg)
\bigg\Vert \bigg] \nonumber \\
& +
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} [\Vert 
\nabla F (\mathbf{w}(\tau_1\tau_2 k_2-1)) - \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\Vert ] \nonumber \\
%%%%        (c)
& \overset{(c)}{\leq}
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\frac{1}{U} \sum_{\hat{u}=1}^{U} \sum_{i=1}^{W_{\hat{u}}} \frac{\Delta_i(k_2)}{\Delta_{\hat{u}}(k_2)}
\mathbb{E} \bigg[\bigg\Vert 
\nabla F_i(\mathbf{w}^{\hat{u}}(\tau_1\tau_2k_2-1)) - \nabla F_i(\mathbf{w}(\tau_1\tau_2k_2-1))
\bigg\Vert \bigg]
\nonumber \\
& +
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\sum_{i=1}^{W_{\hat{u}}} \frac{\Delta_i(k_2)}{\Delta_{\hat{u}}(k_2)} 
\mathbb{E} \bigg[\bigg\Vert 
\nabla F_i(\mathbf{w}(\tau_1\tau_2k_2-1)) - \nabla F_i(\mathbf{w}^{u}(\tau_1\tau_2k_2-1))
\bigg\Vert \bigg] \nonumber \\
& +
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} [\Vert 
\nabla F (\mathbf{w}(\tau_1\tau_2 k_2-1)) - \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\Vert ]  \nonumber \\
%%%%        (d)
& \overset{(d)}{\leq}
\eta_2 \mu_F \frac{1}{U} \sum_{u=1}^{U}
\frac{1}{U} \sum_{\hat{u}=1}^{U} \sum_{i=1}^{W_{\hat{u}}} \frac{\Delta_i(k_2)}{\Delta_{\hat{u}}(k_2)}
\mathbb{E} [\Vert 
\mathbf{w}^{\hat{u}}(\tau_1\tau_2k_2-1) - \mathbf{w}(\tau_1\tau_2k_2-1)
\Vert ]
\nonumber \\
& +
\eta_2 \mu_F \frac{1}{U} \sum_{u=1}^{U}
\sum_{i=1}^{W_{\hat{u}}} \frac{\Delta_i(k_2)}{\Delta_{\hat{u}}(k_2)} 
\mathbb{E} [\Vert 
\mathbf{w}(\tau_1\tau_2k_2-1) - \mathbf{w}^{u}(\tau_1\tau_2k_2-1)
\Vert ] \nonumber \\
& +
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} [\Vert 
\nabla F (\mathbf{w}(\tau_1\tau_2 k_2-1)) - \nabla F_u (\mathbf{w}(\tau_1 \tau_2 k_2 -1))
\Vert ]  \nonumber \\
%%%%        (e)
& \overset{(e)}{\leq}
2\eta_2 \mu_F \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} [\Vert 
\mathbf{w}^{\hat{u}}(\tau_1\tau_2k_2-1) - \mathbf{w}(\tau_1\tau_2k_2-1)
\Vert ]
+
\eta_2 \gamma_F,
\end{align}

\noindent
where $(a)$ introduces $\nabla F_{\hat{u}}(\mathbf{w})$ and $\nabla F_{u}(\mathbf{w})$ terms, $(b)$ uses the triangle inequality followed by the swarm-wide meta-gradient definition from~\eqref{eq:pfl_meta_function_swarm_avg}, $(c)$ applies triangle inequality to the expectations, $(d)$ recalls the $\mu_F$-smoothness property of $\nabla F_i$, and $(e)$ uses the result of Lemma~\ref{theory:lemma_gamma}. Combining~\eqref{eq:prop1_eq7} and~\eqref{eq:prop1_eq8} yields:
\begin{align} \label{eq:prop1_eq9}
& \frac{1}{U}\sum_{u = 1}^{U}
\mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert] \nonumber\\
%%%     (a)
& \overset{(a)}{\leq} 
\frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \frac{1}{U} \sum_{\hat{u} =1}^{U} \mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2 -1)
\bigg\Vert \bigg] \nonumber \\
& +
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} [ \Vert \nabla F_u (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \widetilde{\nabla F_u}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) \Vert ]
\nonumber \\
& + 
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \bigg(
\widetilde{\nabla F_{\hat{u}}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{\hat{u}} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)) 
\bigg)
\bigg\Vert \bigg] 
\nonumber \\
& + 
2\eta_2 \mu_F \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} [\Vert 
\mathbf{w}^{\hat{u}}(\tau_1\tau_2k_2-1) - \mathbf{w}(\tau_1\tau_2k_2-1)
\Vert ]
+
\eta_2 \gamma_F
\nonumber \\
%%%         (b)
& \overset{(b)}{\leq} 
(1+2\eta_2 \mu_F)
\frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \frac{1}{U} \sum_{\hat{u} =1}^{U} \mathbf{w}^{\hat{u}}(\tau_1 \tau_2 k_2 -1)
\bigg\Vert \bigg] + \eta_2 \gamma_F
\nonumber \\
& +
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert 
\sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\bigg(
\nabla F_i (\mathbf{w}^{u}(\tau_1 \tau_2 k_2 -1)) 
- \widetilde{\nabla F_i}(\mathbf{w}^{u}(\tau_1\tau_2 k_2-1)) 
\bigg) \bigg\Vert \bigg] \nonumber \\
& + 
\eta_2 \frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} \bigg[ \bigg\Vert 
\frac{1}{U} \sum_{\hat{u}=1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} \bigg(
\widetilde{\nabla F_{i}}(\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1))
- \nabla F_{i} (\mathbf{w}^{\hat{u}}(\tau_1\tau_2 k_2-1)) 
\bigg)
\bigg\Vert \bigg] 
\nonumber \\
%%%         (c)
& \overset{(c)}{\leq} 
(1+2\eta_2 \mu_F)
\frac{1}{U} \sum_{u=1}^{U}
\mathbb{E} [ \Vert 
\mathbf{w}^{u}(\tau_1 \tau_2 k_2 - 1) - \mathbf{w}(\tau_1 \tau_2 k_2 -1)
\Vert ] + \eta_2 \gamma_F
\nonumber \\
& +
2 \eta_2 \frac{1}{U} \sum_{u=1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2)}{\Delta_u(k_2)} 
\sigma_F^i(\tau_1\tau_2 k_2-1),
\end{align}

\noindent
where $(a)$ combines~\eqref{eq:prop1_eq7} and~\eqref{eq:prop1_eq8}, $(b)$ applies definition of $\nabla F_u$ from~\eqref{eq:pfl_meta_function_swarm_avg}, $(c)$ uses triangle inequality followed by Lemma~\ref{theory:lemma_sigma} and the definition of $\mathbf{w}$ from~\eqref{eq:global_wide_aggregation}.
Solving~\eqref{eq:prop1_eq9} recursively yields:
\begin{align}
\label{eq:prop1_eq10}
& \frac{1}{U}\sum_{u = 1}^{U} \mathbb{E} [ \Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1 \tau_2 k_2) \Vert ] 
\\
& \overset{(a)}{\leq}
2 \eta_2 \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2) }{\Delta_u(k_2)}
\bigg(
\sum_{y=0}^{\tau_1\tau_2-1}\sigma_F^{i}(\tau_1\tau_2 k_2-1-y) (1+2 \eta_2 \mu_F)^{y}
\bigg)
+
\eta_2 \gamma_{F}
\frac{1 - (1+2 \eta_2 \mu_F)^{\tau_1 \tau_2}}{1- (1+2 \eta_2 \mu_F)} \\
& \overset{(b)}{\leq}
\bigg(
2 \eta_2 \frac{1}{U}\sum_{u = 1}^{U}  \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2) }{\Delta_u(k_2)}
\sum_{y=0}^{\tau_1\tau_2-1}\sigma_F^{i}(\tau_1\tau_2 k_2-1-y)
+
\eta_2 \gamma_{F}
\bigg)
\frac{1 - (1+2 \eta_2 \mu_F)^{\tau_1 \tau_2}}{1- (1+2 \eta_2 \mu_F)},
\end{align}
where $(a)$ is the result of recursion and the finite sum of geometric series, and $(b)$ uses $\sum_{i} a_i b_i \leq \sum_{i} a_i \sum_{i} b_i$ $\forall a_i, b_i \geq 0$. Combining the results of~\eqref{eq:prop1_eq6} and~\eqref{eq:prop1_eq10} in~\eqref{eq:prop1_eq2} yields:
\begin{equation}
\label{eq:prop1_eq14}
\begin{aligned}
& \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2) }{\Delta_u(k_2)}
\bigg( \mathbb{E}[\Vert \mathbf{w}^{i}(\tau_1\tau_2 k_2) - \mathbf{w}^{u}(\tau_1\tau_2 k_2) \Vert ] + \mathbb{E}[\Vert \mathbf{w}^{u}(\tau_1\tau_2 k_2) - \mathbf{w}(\tau_1\tau_2 k_2)
\Vert] \bigg) \\
& \leq 
\bigg(
2 \eta_2 \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2) }{\Delta_u(k_2)}
\sum_{y=1}^{\tau_1}
\sigma_F^{i}(\tau_1 \tau_2 k_2 - y)
+
\eta_2
\frac{1}{U} \sum_{u = 1}^{U}\gamma_{F}^{u}
\bigg)
\frac{1 - (1+2 \eta_2 \mu_F)^{\tau_1}}{1- (1+2 \eta_2 \mu_F)}\\
& +
\bigg(
2 \eta_2 \frac{1}{U}\sum_{u = 1}^{U} \sum_{i = 1}^{W_u} \frac{\Delta_i(k_2) }{\Delta_u(k_2)}
\sum_{y=1}^{\tau_1\tau_2}\sigma_F^{i}(\tau_1\tau_2 k_2-y)
+
\eta_2 \gamma_{F}
\bigg)
\frac{1 - (1+2 \eta_2 \mu_F)^{\tau_1 \tau_2}}{1- (1+2\eta_2 \mu_F)},
\end{aligned}
\end{equation}
with the summation shifted from $y=0$ to $y=1$.
\end{proof}
